Lazy Abstraction-Based Controller Synthesis

We present lazy abstraction-based controller synthesis (ABCS) for continuous-time nonlinear dynamical systems against reach-avoid and safety specifications. State-of-the-art multi-layered ABCS pre-computes multiple finite-state abstractions of varying granularity and applies reactive synthesis to the coarsest abstraction whenever feasible, but adaptively considers finer abstractions when necessary. Lazy ABCS improves this technique by constructing abstractions on demand. Our insight is that the abstract transition relation only needs to be locally computed for a small set of frontier states at the precision currently required by the synthesis algorithm. We show that lazy ABCS can significantly outperform previous multi-layered ABCS algorithms: on standard benchmarks, lazy ABCS is more than 4 times faster.

==> Preliminaries.tex <==
\section{Control Systems and the Control Problem}\label{sec:prelim}

% We first recall necesseary notations and constructions for multi-layered ABCS using FRR as developed in \cite{hsu2018multi} based upon \cite{ReissigWeberRungger_2017_FRR}.


\smallskip
\noindent\textbf{Notation.}
Given $a,b\in\real{}\cup\set{\pm\infty}$ with $a\leq b$, we denote by $[a,b]$ the closed interval $\set{s\in\real{}\mid a\leq x\leq b}$.
For a vector $a\in(\real{}\cup\set{\pm\infty})^n$ and $i\in\set{1,\ldots, n}$, we denote the $i$th component of $a$ by $a_{i}$.
We define the relations $<,\leq,\geq,>$ on vectors in $\real{n}$ component-wise.

For a set $A$, we write $A^*$ and $A^\infty$ for the set of finite, and the set of finite or infinite sequences over $A$, respectively.
For $w\in A^*$, we write $|w|$ for the length of $w$; the length of an infinite sequence is $\infty$. 
For $0 \leq k < |w|$ we write $w(k)$ for the $k$-th symbol of $w$.

\smallskip
\noindent\textbf{Continuous-Time Control Systems.}\
A \emph{control system} $\Sigma = (X, U, W, f)$
consists of a state space $X= \real{n}$, a non-empty input space $U\subseteq\real{m}$, 
a compact disturbance set $W\subset \real{n}$ with $0\in W$, and 
a function $f:X\times U\rightarrow X$ s.t. $f(\cdot,u)$ is locally Lipschitz for all $u\in U$. 
%
Given an initial state $x_0\in X$, a positive parameter $\tau>0$, and a constant input trajectory $\mu_u:[0,\tau]\rightarrow U$
which maps every $t\in [0,\tau]$ to the same $u\in U$, 
a \emph{trajectory} of $\Sigma$ 
on $[0,\tau]$ is an absolutely continuous function $\xi:[0,\tau]\rightarrow X$  s.t. $\xi(0) = x_0$ and
$\xi(\cdot)$ fulfills the following differential inclusion for almost every $t\in[0,\tau]$:
\begin{equation}\label{equ:def_f}
 \dot{\xi}\in f(\xi(t),\mu_u(t))+W = f(\xi(t),u) + W. 
\end{equation} 
We collect all such solutions in the set $\ON{Sol}_f(x_0,\tau,u)$. 


\smallskip
\noindent\textbf{Control Problem.}\
\RM{is there a way to define a controller for the original control system? define closed loop?}
We shall consider the behaviors of a control system within a compact \emph{region of interest} $Y \subseteq X$, and our
goal will be to synthesize a dynamic controller which ensures a given temporal specification within $Y$.
Thus, we interpret $Y$ as a \emph{global safety requirement} 
and synthesize a controller which keeps the system within $Y$ while implementing a temporal specification.

We shall consider two temporal specifications: (a) safety control and (b) reach-avoid control.
We assume we are given a set of \emph{goal states} $\goal\subseteq Y$ and a set of \emph{static obstacles} $\obstacle \subset X$.
Safety control asks to find a controller such that all trajectories of the closed loop system
always remain within the set $\Rset = Y \setminus \obstacle)$ of \emph{safe states}.
Reach-avoid control asks that all trajectories eventually visit some state in the target $\Tset=\goal\cap \Rset$
while always remaining within $\Rset$. 
These specifications are formalized in linear temporal logic (LTL) \cite{baier2008principles} as: 
%
\begin{subequations}\label{equ:LTLspec}
\begin{align}
	\Specs &= \text{always}\; (\Rset{}),\quad\text{and}\label{equ:LTLspec:safe}\\
	\Specr &= \left[\left(\text{always}\; (\Rset )\right)\; \text{until} \; T\right] \wedge \left[\text{eventually}\; T\right],\label{equ:LTLspec:reach}
\end{align}
\end{subequations}
\RM{why the eventually T?}
respectively, where we interpret the sets $T$ and $R$ as predicates over the state space.
% Intuitively, the specification asks the system to stay within $R$, and, in the case of reach-avoid control, to additionally enforce a visit to the target $T$. 
We refer to these control problems for a given dynamical system $\Sigma$ jointly as $\tuple{\Sigma,\Spec}$.
% 
The goal of this paper is to compute a controller which solves a control problem $\tuple{\Sigma,\Spec}$, 
i.e., which ensures that, when connected to $\Sigma$ in feedback, all trajectories of the resulting closed loop fulfill the respective 
LTL properties in \eqref{equ:LTLspec}.



\section{Abstract Systems}
\label{sec:abstract-system}

\smallskip
\noindent\textbf{Time-Sampled System.}\
Given a time sampling parameter $\tau>0$, we define the \emph{time-sampled system} $\St{}(\Sigma,\tau)=(X,U,\Ft{})$ associated with $\Sigma$, 
where $X$, $U$ are as in $\Sigma$, and the transition function $\Ft{}:X\times U\fun 2^X$ is defined as follows.
For  all $x\in X$ and $u \in U$, we have $x'\in \Ft{}(x,u)$ iff there exists a solution $\xi\in\ON{Sol}_f(x,\tau,u)$ s.t.\ $\xi(\tau)=x'$.

\smallskip
\noindent\textbf{Covers and Grid-aligned Covers.}\ 
For vectors $a,b\in(\real{}\cup\Set{\pm\infty})^n$, a \emph{cell} $\hyint{a,b}$ is the semi-open set $\set{x\in\real{n}\mid \forall i\in\set{1,\ldots,n}.a_i\leq x_i < b_i}$.
A \emph{cover} $\hat{X}$ of  $X$ is a finite set of non-empty and non-overlapping cells 
$\hyint{a,b}$ with $a,b\in (\real{}\cup\Set{\pm\infty})^n$, s.t.\ every $x\in X$ belongs to exactly one cell $\xa\in\hat{X}$. 

Let $\eta \in\real{}_{>0}^n$ be a parameter.
We shall consider the behaviors of a control system within a compact
\emph{region of interest}
$Y = \hyint{\alpha, \beta}$, where $\alpha,\beta\in\real{n}$ and \RM{do we need it here?}
$\beta - \alpha$ is an integer multiple of $\eta$.
\RM{also a multiple of $2\eta$, $4\eta$, etc}
A point $c\in Y$ is \emph{$\eta$-grid-aligned} if there is $k\in\Z^n$ s.t.\ for each $i\in \set{1,\ldots,n}$,
$c_i = \alpha_i + k_i\eta_i - \frac{\eta_i}{2}$.
A cell $\hyint{a,b}$ is \emph{$\eta$-grid-aligned} if there is a $\eta$-grid-aligned point $c$ s.t.\ $a = c - \frac{\eta}{2}$ and
$b = c + \frac{\eta}{2}$;
such cells define sets of diameter $\eta$ whose center-points are $\eta$-grid-aligned. 
Clearly, the set of $\eta$-grid-aligned cells is a \emph{finite cover} for $Y$.

In the following, we assume the region of interest $Y$ is fixed once and for all.
\RM{OMIT?}\footnote{
	$Y$ induces a \emph{finite} \RM{undef:} abstaction by restricting attention to a subset of the state space for control. 
	$Y$ can also be interpreted as a global safety requirement (see Sec.~\ref{sec:problem}).}

\smallskip
\noindent\textbf{Abstract Systems.}\ 
An \emph{abstract system} $\Sa{}(\Sigma,\tau,\eta)=(\Xa{},\Ua{},\Fa{})$ for a control system $\Sigma$,
a time sampling parameter $\tau > 0$, and a grid parameter $\eta \in \real{n}_{>0}$
consists of:
% 
\begin{inparaenum}[(i)]
 \item an abstract state space $\Xa{}$ which forms a finite cover of $X$;
 moreover, we assume there is a non-empty subset 
 $\Ya{}\subseteq\Xa{}$ which forms a finite cover of $Y$ with $\eta$-grid aligned cells,
 \item a finite abstract input space $\Ua\subseteq U$, and
 \item an abstract transition function 
$\Fa{}:\Xa{}\times \Ua{}\rightarrow 2^{\Xa{}}$ such that 
for all $\xa\in(\Xa{}\setminus\Ya{})$ and $u\in\Ua$ we have $\Fa{}(\xa,u)=\emptyset$ 
and for all $\xa\in\Ya{}$, $\xa'\in\Xa{}$, and $u\in\Ua{}$ 
it holds that
 \begin{align}\label{eq:next state abs sys 0}
   \xa'\in \Fa{}(\xa,u) \ \mbox{ if } \ 	\exists\xi\in \cup_{x\in\xa}\ON{Sol}_f(x,\tau,u) \;.\; \xi(\tau) \in \xa'.
 \end{align}
\end{inparaenum}
We extend $\Fa{}$ to sets of abstract states $\Upsilon\subseteq \Xa{}$ by defining $\Fa{}(\Upsilon,u) := \bigcup_{\xa\in \Upsilon} \Fa{}(\xa,u)$.


We consider multiple abstract systems obtained in this way.
For parameters $\n{1} > 0$ and $\ta{1} >0$, 
and for $l\in\mathbb{Z}_{>1}$, we define $\n{l} = 2\n{l-1}$ and $\ta{l} = 2\ta{l-1}$.
With this, we obtain a sequence of $L$ time-sampled and abstract systems
\begin{align}\label{equ:StsetSaset}
 \Stset:=\set{\St{l}(\Sigma,\ta{l})}_\layer\quad \text{and}\quad \Saset:=\set{\Sa{l}(\Sigma,\ta{l},\n{l})}_\layer,
\end{align}
respectively, where\footnote{If $\Sigma$, $\tau$, and $\eta$ are
clear from the context, we omit them in $\St{l}$ and $\Sa{l}$.} $\St{l}:=(X,U,\Ft{l})$ and $\Sa{l}:=(\Xa{l},\Ua{},\Fa{l})$.
% 

% \begin{figure}[t]
% 	\centering
% 	\input{Figures/growth_bound}
% 	\caption{Computation of abstract transitions based on a growth bound: the gray box is the abstract state $\xa$, the blue box is the over-approximation of the set of states reachable from $\xa$ using some control input $u$, and the $4$ cells covered with hatch-lines constitute the set $\Fa{}(\xa,u)$.}
% 	\label{fig:growth bound}
% \end{figure}

% We also extend the notation of $\Fa{}$ to work on sets of abstract states: for any $\Xa{}'\subseteq \Xa{}$, $\Fa{}(\Xa{}',u) = \bigcup_{\xa\in \Xa{}'} \Fa{}(\xa,u)$. 
As the exact computation of $\cup_{x\in\xa}\ON{Sol}_f(x,\tau,u)$ in \eqref{eq:next state abs sys 0} is expensive (if not impossible), a numerical over-approximation is usually computed instead.
We assume that the latter is monoton in the granularity of the discretization.
\begin{assumption}\label{assumption:monotonic approximation}
Let $\Sa{l}$ and $\Sa{m}$ be two abstract systems with $m,\layer$, $l<m$. Then\footnote{We write $\Upsilon_{l}\subseteq \Upsilon_{m}$ with $\Upsilon_{l}\subseteq \Xa{l}$, $\Upsilon_{m}\subseteq \Xa{m}$ as short for $\bigcup_{\xa\in \Upsilon_l}\xa\subseteq \bigcup_{\xa\in \Upsilon_m}\xa$.} $\Fa{l}(\Upsilon_l) \subseteq \Fa{m}(\Upsilon_m)$ if $\Upsilon_{l}\subseteq \Upsilon_{m}$.
% 	and $\Sa{2}(\Sigma,\tau,\eta_2)=(\Xa{2},\Ua{},\Fa{2})$ be two abstract systems with $\eta_1 < \eta_2$.
% 	Let $\Upsilon_1 \subset \Xa{1}$ and $\Upsilon_2\subset \Xa{2}$ be sets of states s.t.\ $\Upsilon_{l}\subseteq \Upsilon_{m}$.
% 	Then, we assume that $\Fa{1}(\Upsilon_1) \subseteq \Fa{2}(\Upsilon_2)$.
\end{assumption} 
Assumption~\ref{assumption:monotonic approximation} is fulfilled by many reachable set approximation methods e.g.\ based on decomposition functions for mixed-monotone systems \cite{coogan2015efficient} or on growth bounds \cite{ReissigWeberRungger_2017_FRR,Scots}, as used by our implementation.
%Notice that $T$ is not used in this definition, but will be used in our algorithms.


\smallskip
\noindent\textbf{Feedback Refinement Relations.} 
A relation $\Qa{}\subseteq X\times \Xa{}$ 
is called a \emph{feedback refinement relation (FRR)} \cite{ReissigWeberRungger_2017_FRR} from $\St{}$ to $\Sa{}$, 
written $\St{}\frr{\Qa{}}\Sa{}$, if for all $(x,\xa)\in \Qa{}$ we have
\begin{inparaenum}[(i)]
 \item $U_{\Sa{}}(\xa)\subseteq U_{\St{}}(x)$, and 
 \item $u\in U_{\Sa{}}(\xa) \Rightarrow \Qa{}(\Ft{}(x,u))\subseteq \Fa{}(\xa,u)$,
\end{inparaenum}
 where $U_{\St{}}(x):=\SetComp{u\in U}{\Ft{}(x,u)\neq \emptyset}$ and $U_{\Sa{}}(x):=\SetComp{u\in U}{\Fa{}(x,u)\neq \emptyset}$. 
 It can be shown that the relation $\Qa{}:=\{(x,\xa) \in X\times \Xa{} \mid x\in \xa\}$ is a (canonical) feedback refinement relation from $\St{}$ to $\Sa{}$ \cite{ReissigWeberRungger_2017_FRR}. 
  
% \ $(x,\xa)\in\Qa{}$ iff $x\in\xa$ and for each $x$ exists some $\xa$ such that $(x,\xa)\in \Qa{}$. Then $\Qa{}$ is a \emph{feedback refinement relation (FRR)} from $\St{}$ to $\Sa{}$ 
%written $\St{}\frr{\Qa{}}\Sa{}$ (see ).
% 

For sequences of time-sampled and abstract systems $\Stset$ and $\Saset$ from \eqref{equ:StsetSaset}, we have a sequence $\{\Qa{l}\}_\layer$ of (canonical) FRRs between the corresponding systems which induce relations $\Ra{ll'}\subseteq\Xa{l'}\times\Xa{l}$ for 
$1\leq l$, $l'\leq L$ between abstract states of different layers such that%
\footnote{We also use $\Qa{}$ and $\Ra{}$ as functions and extend them to sets of states.}
\begin{align}\label{equ:Ra}
 \propAequ{\xa\in\Ra{ll'}(\xa')}{\xa\in \Qa{l}(\Qai{l'}(\xa')).}
\end{align}
% 
However, the relation $\Ra{ll'}$ is generally \emph{not} a FRR between the layers (see \cite{hsu2018multi}, Rem. 1). 
This means that $\Sa{l+1}$ cannot be directly constructed from $\Sa{l}$, unlike in usual abstraction refinement algorithms \cite{ClarkeGJLV03,henzinger2002lazy,AlfaroRoy_2010}.



% 
% 
% 
% To map abstract states between different layers of abstraction, we use the operator 
% 	\begin{equation}\label{equ:Gamma}
% 	 		\UA{ll'}(\Upsilon_{l'}) = 
% 			\begin{cases}
% 				\Ra{ll'}(\Upsilon_{l'}), & l \leq l' \\
% 				\SetComp{\hat{x} \in \Xa{l}}{\Ra{l'l}(\hat{x})\subseteq \Upsilon_{l'}}, & l > l' 
% 			\end{cases}
% 	\end{equation}
% and its dual
% \begin{align}\label{eq:def over approx}
% 	\OA{ll'}(\Upsilon_{l'}) := \begin{cases}
% 								\Ra{ll'}(\Upsilon_{l'}), & l \leq l' \\
% 								\SetComp{\hat{x} \in \Xa{l}}{\Ra{l'l}(\hat{x})\cap \Upsilon_{l'} \neq \emptyset}, & l > l' 
% 							\end{cases}
% \end{align}
% where $l,l'\in [1;L]$ and $\Upsilon_{l'}\subseteq \Xa{l'}$. 
% The operations $\UA{ll'}(\Upsilon_{l'}) \subseteq \Xa{l}$ (resp. $\OA{ll'}(\Upsilon_{l'}) \subseteq \Xa{l}$)  under(resp. over-) approximate a set $\Upsilon_{l'} \subseteq \Xa{l'}$ with one in layer $l$. 

 \smallskip
 \noindent\textbf{Controllers and Closed Loop Systems.}
 %\label{sec:prelim:Control}
 %
 We model a \emph{controller} as a function $\Gc$ that maps system states to control inputs.
 The controller is represented by the triple $\C=(\Uc,\Yc,\Gc)$, where $\Uc$ is the controller domain, $\Yc$ is the controller image, and $\Gc:\Uc\fun 2^{\Yc}$ is the control map of $\C$.
 % 
 We say that $\C=(\Uc,\Yc,\Gc)$ is \emph{composable} with $\Sa{}=(\Xa{},\Ua,\Fa{})$ 
 if
 % \footnote{
 % 	In \cite{ReissigWeberRungger_2017_FRR} a system is feedback composable with a controller if $X\subseteq \Uc$. 
 % 	We invert this relationship; we consider controllers whose domain is only a subset of the system's state 
 % 	space and assume that controllers do not have other inputs.}
 $\Uc\subseteq \Xa{}$ and $\Yc\subseteq \Ua$. 
 For notational simplicity, we only consider controllers with $\Yc=\Ua$.
 % 
 The \emph{closed loop system} formed by interconnecting
 $\Sa{}$ and $\C$ in \emph{feedback} 
 is defined by the system 
 $\Sa{}^{cl}=(\Xa{}, \Fa{}^{cl})$ with $\Fa{}^{cl}:\Xa{}\fun 2^{\Xa{}}$ s.t.\ 
 $\xa'\in\Fa{}^{cl}(\xa)$ iff there exists $\ua\in\Gc(\xa)$ s.t.\ $\xa'\in\Fa{}(\xa,\ua)$.
 % \KM{What is the purpose of having $B$ in the description of the closed loop (in Anne's version)? In any case, if $B$ is there, we need to update $B$ with the state evolution of the system as otherwise the closed loop will get stuck. I removed $B$.}
 
 As $\St{}\frr{Q} \Sa{}$, it follows from \cite{ReissigWeberRungger_2017_FRR} that a controller $\C$ composable with $\Sa{}$ can be \emph{refined} into a controller composable with $\St{}$ via $Q$. 
 This is formalized using the closed loop system $\St{}^{cl}=(X, \Ft{}^{cl})$ with $\Ft{}^{cl}:X\fun 2^X$ s.t.\ for any state $x\in X$, $\Ft{}^{cl}(x) := \Ft{}(x,G\circ Q(x))$.
%  
The behavior $\Behtcl{}$ of $\St{}^{cl}$ contains all trajectories $\xi\in X^\infty$ with are compatible with $\St{}^{cl}$, i.e., for all $1\leq k < |\xi|$ holds that $\xi(k)\in \Ft{}^{cl}(\xi(k-1))$, and maximal, i.e., if $|\xi| < \infty$ it holds that $\\Ft{}^{cl}(\xi(|\xi|))= \emptyset$.
% % ***** New version ****
% \begin{equation}
%  \Behtcl{} := \SetComp{\xi\in X^\infty}{\left(|\xi| < \infty \Rightarrow \Ft{}^{cl}\left(\xi(|\xi|)\right) = \emptyset\right) \wedge\left( \AllQ{1\leq k < |\xi|}{\xi(k)\in \Ft{}^{cl}(\xi(k-1))}\right)}.
% \end{equation}
The behavior $\Behacl{}$ of $\Sa{}^{cl}$ is defined analogously via $\Fa{}^{cl}$. Note that all finite traces contained in $\Behtcl{}$ and $\Behacl{}$ are by definition blocking.

% Similar to the closed loop trajectories of the sampled-time system, we also define the closed loop trajectory of the abstract system:
% $\Behacl{} := \textstyle\SetComp{\xia\in \Xa{}^\infty}{\left(|\xia| < \infty \Rightarrow \Fa{}^{cl}\left(\xia(|\xia|)\right) = \emptyset\right) \wedge\left( \AllQ{1\leq k < |\xia|}{\xia(k)\in \Fa{}^{cl}(\xia(k-1))}\right)}.$
 

\smallskip
\noindent\textbf{Multi-Layered Controllers and Closed Loops.}
Given a multi-layered abstract system $\Saset$ and some $P\in \mathbb{N}$, a multi-layered controller  $\Cset=\set{\Ci{p}}_{\controllers}$ with $\Ci{p}=(\Uci{p}, \Ua,\Gci{p})$ and $\Gci{p}:\Uci{p}\fun 2^{\Ua}$ is composable with $\Saset$ if for all $\controllers$ there exists a unique $\li\in[1;L]$ s.t.\ $\Ci{p}$ is composable with $\Sa{\li}$, i.e., $\Uci{p}\subseteq \Xa{\li}$. We denote by $\dom{\Cset}=\bigcup_\controllers\Uci{p}$ the domain of $\Cset$.
% We denote by $\dom{\Ci{p}}=\Uci{p}$ the domain of $\Ci{p}$.
%  
The number $P$ is not necessarily related to $L$; we allow for multiple controllers to be composable with the same layer and no controller to be composable for some layers. %; formally, there might exist $p,q\in[1;P]$, $p\neq q$, s.t. $\li=l_{q}$, and there might exist \layer s.t.\ there exists no \controllers s.t. $\li=l$.

The \emph{quantizer induced by $\Cset$} is defined as the 
map $\Qset:X\fun 2^{\Xaall}\setminus\set{\emptyset}$ with $\Xaall=\bigcup_\layer \Xa{l}$ s.t.\ for all $x\in X$ it holds that $\xa\in\Qset(x)$ iff either
\begin{compactenum}[(i)]
 \item there exists $p\in[1;P]$ s.t.\  $\xa\in\Qa{l_p}(x)\cap\Uci{p}$
 and no $p'\in[1;P]$ s.t.\ $l_{p'}>l_p$ and $\Qa{l_{p'}}(x)\cap\Uci{p'}\neq\emptyset$,
or 
 \item $\xa\in\Qa{1}(x)$ and $\xa\notin\Qa{l_{p}}(x)\cap\Uci{p}$ for all $p\in[1;P]$.
\end{compactenum}
% 
% \KM{Why should the output of $\Qset$ be ever be a set if we follow this definition? I think $\Qset:X\rightarrow \Xa{}$, because for any given $x\in X$, $\Qset$ maps $x$ to an unique abstract state. No?}
% We identify $\Qset$ with the map $\Qset_z:X\fun 2^{\Xaall}$ s.t.\ $\xa\in \Qset_z(x)$ iff $(\xa,z)\in\Qset (x,z)$. 
We define $\img{\Qset}=\SetComp{\xa\in\Xaall}{\ExQ{x\in X}{\xa\in\Qset(x)}}$. %If $\Cset$ is strict, $\Qset_z$ is simply denoted by $\Qset$. 
% 
In words, $\Qset$ maps states $x\in X$ to the \emph{coarsest} abstract state $\xa$ that is both related to $x$ and is in the domain of $\Cset$ (condition (i)). If such an abstract state does not exist, $\Qset$ maps $x$ to its related layer $l=1$ states (condition (ii)).
% $\Qa{l}$ is non-deterministic for states which lie at the boundary of two cells $\xa,\xa'\in\Xaall{l}$. If such an $x$ happens to be located at the boundary of controller domains computed for different layers, $\Qset_z$ maps $x$ to two abstract cells within different layers.

The \emph{closed loop system} formed by interconnecting
$\Saset$ and $\Cset$ in \emph{feedback} 
is defined by the system 
$\Saset^{cl}=(\Xaall, \Faall^{cl})$ with $\Faall^{cl}:\img{\Qset}\fun2^{\img{\Qset}}$ s.t.\ 
$\xa'\in\Faall^{cl}(\xa)$ iff there exists $p\in[1;P]$, $\ua\in\Gci{p}(\xa)$ and $\xa''\in\Fa{\li}(\xa,\ua)$ s.t.\ $\xa'\in\Qset(\Qai{\li}(\xa''))$.
% 
%\new{
%As $\St{l}\frr{\Qa{l}} \Sa{l}$ for all $l\in[1;L]$, we can obtain a controller for $\Stset$ by first quantizing the state $x$ of $\Stset$ into a state $\xa$ of $\Saset$ using $\Qset$, and then applying $\Cset$ on $\xa$ to find the respective control input.
%This process is called controller \emph{refinement} (see \cite{hsu2018multi}, Sec.~3.4).
%}
This results in the closed loop system
$\Stset^{cl}=(X, \Ftall^{cl})$ with $\Ftall^{cl}:X\fun 2^X$ s.t.\
$x'\in\Faall^{cl}(x)$ iff there exists $\xa\in \Qset(x)$, $p\in[1;P]$ and $\ua\in\Gci{p}(\xa)$ s.t.\ $x'\in\Fa{\li}(x,\ua)$.
% 
Similar to $\Behtcl{}$ and $\Behacl{}$, we define $\Behtclset$ and $\Behaclset$ by replacing $\Ft{}^{cl}$ and $\Fa{}^{cl}$ with $\Ftall^{cl}$ and $\Faall^{cl}$ respectively.
%The behavior of $\Stset^{cl}$ is defined by 
% ***** New version ****
%\new{
%$\Behtclset := \textstyle\SetComp{\xi\in X^\infty}{\left(|\xi| < \infty \Rightarrow \Ftall^{cl}\left(\xi(|\xi|)\right) = \emptyset\right) \wedge\left( \AllQ{1\leq k < |\xi|}{\xi(k)\in \Ftall^{cl}(\xi(k-1))}\right)}.$
%Note that all the finite traces in $\Behtclset $ are by definition blocking behaviors of $\Stset^{cl}$.}
%\label{equ:def:Behtcl}}%\\
% ***** Old version *****
% $
% \Behtclset:=\textstyle\SetComp{\xi\in X^\infty}{\AllQ{1\leq k < |\xi|}{\xi(k)\in \Ftall^{cl}(\xi(k-1))}}%\label{equ:def:Behtcl}}%\\
% %\Behaclset&:=\textstyle\SetComp{\xia\in \Xaall^\infty}{\AllQ{1\leq k < {|\xia|}}{\xia(k)\in \Faall^{cl}(\xia(k-1))}}.%\label{equ:def:Behacl}
%$.
% ***** end: old version ****
Note that, %$\Behaclset$ contains trajectories composed from abstract states of different coarseness and 
$\Behtclset$ contains trajectories with non-uniform sampling time.

%\new{
%Similar to the closed loop trajectories of the sampled-time system, we also define the closed loop trajectory of the abstract system:
%$\Behaclset := \textstyle\SetComp{\xia\in \Xa{}^\infty}{\left(|\xia| < \infty \Rightarrow \Faall^{cl}\left(\xia(|\xia|)\right) = \emptyset\right) \wedge\left( \AllQ{1\leq k < |\xia|}{\xia(k)\in \Faall^{cl}(\xia(k-1))}\right)}.$}


==> ProblemStatement.tex <==
\section{Problem Formulation}\label{sec:problem}

When constructing the abstract transition system $\Sa{}$ of a dynamical system $\Sigma$ for ABCS we used a global region of interest $Y\subseteq X$ to ensure \emph{finiteness} of the abstraction for controller synthesis. As this implies that the resulting controller is only valid within $Y$, we interpret $Y$ as a \emph{global safety requirement} and synthesize a controller which keeps the system within $Y$ while implementing the actual specification, i.e., safety or reachability in our case.
To formalize these control problems, we consider a given set of \emph{goal states} $G\subseteq Y$ and \emph{static obstacles} $O \subset X$ inducing a set of safe states $\Rset=Y\setminus O$ and target states $\Tset=G\cap\Rset$. Given these sets we consider two different scenarios: (a) safety control and (b) reach-avoid control\footnote{We consider a reach-avoid specification instead of a pure reachability problem to ensure the global safety requirement $Y$. As a by-product, this allows to handle additional obstacles $O$ within $Y$ during reachability control. }, formalized in linear temporal logic (LTL) \cite{baier2008principles} as: 
\begin{subequations}\label{equ:LTLspec}
\begin{align}
	\Specs &= \text{always}\; (\Rset{}),\quad\text{and}\label{equ:LTLspec:safe}\\
	\Specr &= \left[\left(\text{always}\; (\Rset )\right)\; \text{until} \; T\right] \wedge \left[\text{eventually}\; T\right],\label{equ:LTLspec:reach}
\end{align}
\end{subequations}
respectively, where we interpret the sets $T$ and $R$ as predicates over the state space.
Intuitively, the specification asks the system to stay within $R$, and, in the case of reach-avoid control, to additionally enforce a visit to the target $T$. We refer to these control problems for a given dynamical system $\Sigma$ jointly as $\tuple{\Sigma,\Spec}$.
% 
The goal of this paper is to compute a controller which solves a control problem $\tuple{\Sigma,\Spec}$, i.e., which ensures that, when connected to $\Sigma$ in feedback, all trajectories of the resulting closed loop fulfill the respective LTL property in \eqref{equ:LTLspec}.

Towards this goal, we apply the standard framework for grid-based ABCS using FRR \cite{ReissigWeberRungger_2017_FRR} which was transferred to the multi-layered case in \cite{hsu2018multi}. 
Here, one first computes a discrete multi-layered controller $\Cset$ for the multi-layered abstract transition system $\Saset{}$ obtained from $\Sigma$ w.r.t.\ $\Spec$.
We introduce the notation $\WIN(\Saset{},\Spec)$ as the set of all multi-layered controllers $\Cset$ for $\Saset{}$, s.t.\ $\Spec$ holds for all the trajectories $\xia\in\Behaclset$ of the closed loop formed by $\Cset$ and $\Saset{}$ (see more details on the construction of this closed loop at the end of \REFsec{sec:prelim}).
% using 
% \emph{unter-approximations} of $R$ and $T$ by $\Rseta{l},\Tseta{l}\subseteq\Ya{l}$ for every \layer s.t.\
% \begin{align}
%  \Rseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}},~\text{and}~
%  \Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset{}}.
% \end{align}
% I.e., for any $\xia(k)$ we have that whenever it is a layer $l$ cell which is currently the largest cell in the domain of $\Cset$, then it must be contained in the under-approximation $\Rseta{l}$ of the safe set for this layer, and, if reach-avoid control is considered, there need to exists a $k'$ s.t.\ $\xia(k')$ is contained in the under-approximation $\Tseta{l}$ of $T$, where
% $\Rseta{l},\Tseta{l}\subseteq\Ya{l}$ are defined for every \layer s.t.\
% \begin{align}
%  \Rseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}},~\text{and}~
%  \Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset{}}.
% \end{align}
%  \eqref{equ:Csetsound:reach} can be interpreted analogously.
% 
It is the main property of ABCS (see \cite{hsu2018multi}, Sec.~3.4 for a formal proof) that any such abstract controller $\Cset\in\WIN(\Saset{},\Spec)$ can then be applied to the time-sampled system $\Stset{}$ via the FRR $\Qset$ which is ensured to hold layer-wise between every $\St{l}$ and $\Sa{l}$ by construction (see \REFsec{sec:prelim} for details). Intuitively, this results in a sample-and-hold controller with non-uniform sampling time for $\Sigma$ which ensures that $\Spec$ holds on all closed-loop trajectories \emph{at sampling instances}%
\footnote{This implicitly assumes that sampling times and grid sizes are such that no \enquote{holes} occur between consecutive cells visited by a trajectory. This can be formalized by assumptions on the growth rate of $f$ in \eqref{equ:def_f} which is beyond the scope of this paper.
% 
% Note that for multi-layered control, considered sampling instances might be non-uniformly spaced.
}.
% 
% 
% Formally, this classical result of ABCS using FRR (see \cite[Sec.VI.A]{ReissigWeberRungger_2017_FRR}) which was transferred to the multi-layered case in \cite{HsuMajumdarMallikSchmuck_HSCC18}, Sec.~3.4, states that a multi-layered controller $\Cset$ solves $\tuple{\Sigma,\Spec}$ \emph{at sampling instances} when refined via $\Qset$, denoted by $\Cset\in\WIN(\Sigma,\Spec)$, if 
% $\Spec$ holds for all trajectories $\xia\in\Behaclset$  of the closed loop formed by $\Cset$ and $\Saset{}$ (see more details on the construction of this closed loop at the end of \REFsec{sec:prelim})

% 
% \begin{subequations}\label{equ:Csetsound}
%  \begin{align}
%  &\AllQ{\xia\in\Behaclset,k\in\dom{\xia}}{\Qset^{-1}(\xia(k))\in\Rset{}},~\text{and}\label{equ:Csetsound:safe}\\
%  &\AllQ{\xia\in\Behaclset}{\ExQ*{k\in\dom{\xia}}{
%  \begin{propConjA}
%   \Qset^{-1}(\xit(k))\in\Tset{}\\
%   \AllQ{k' \leq k}{\Qset^{-1}(\xit(k'))\in \Rset{}}
%  \end{propConjA}
%  }},\label{equ:Csetsound:reach}
% \end{align}
% \end{subequations}
% respectively.
% When considering \emph{unter-approximations} of $R$ and $T$ by $\Rseta{l},\Tseta{l}\subseteq\Ya{l}$ for every \layer s.t.\
% \begin{align}
%  \Rseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}},~\text{and}~
%  \Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset{}},
% \end{align}
% the right side of \eqref{equ:Csetsound:safe} states that $\xia(k)\in\img{\Qset}\cap\Xa{l}$ implies $\xia(k)\in\Rseta{l}$. That is, if $\xia(k)$ is a layer $l$ cell which is currently the largest cell in the domain of $\Cset$, then it must be contained in the under-approximation $\Rseta{l}$ of the safe set for this layer.  \eqref{equ:Csetsound:reach} can be interpreted analogously.

A multi-layered controller $\Cset\in\WIN(\Saset{},\Spec)$ is typically not unique; there can be many different control strategies implementing the same specification. However, the largest possible controller domain for a particular abstraction layer $l$ always exists and is unique. %, because the winning regions (any set of states which is inside the domain of some controller in $\WIN(\Sigma,\Spec)$) are closed under set union by definition. 
In this paper we will compute a controller  $\Cset\in\WIN(\Saset{},\Spec)$ with a maximal domain w.r.t.\ the lowest layer $l=1$, i.e., if the domain of all controllers $C^p\in\Cset$ are projected to $l=1$, their union is equivalent to the maximal controller domain resulting from synthesis over $\Sa{1}$ only. On top of that, we ensure that cells within this domain are only refined if needed. 
% We call controllers fulfilling this requirement \emph{maximal}.


% and (b) using maximal cell sizes within this domain. I.e., there exists no other multi-layered controller $\Cset'\in\WIN(\Sigma,\Spec)$ with (a) a larger domain or (b) larger cells throuout its domain. We call controllers fulfilling this requirement \emph{maximal}.

% if for all $\xit\in\Behtclset$ it holds that $\xit(k)\in\Rset{}$ for all $k\in\dom{\xit}$.
% Similarely,  $\Cset$ solves a reach-avoid control problem $\tuple{\Sigma,\Specr}$ if for all $\xit\in\Behtclset$ exists a \emph{finite} $k\in\dom{\xit}$ s.t.\ $\xit(k)\in\Tset{}$, and for all $k' \leq k$, $\xit(k')\in \Rset$. 
%  
% By adopting a classical result of ABCS using FRR (see \cite[Sec.VI.A]{ReissigWeberRungger_2017_FRR}) to the multi-layered case (see \cite{HsuMajumdarMallikSchmuck_HSCC18}, Sec.~3.4) we know that for any $\Cset\in\WIN(\Sigma,\Spec)$ equation \eqref{equ:Csetsound} equivalently holds for abstracts state trajectories $\xia\in\Behaclset$  of the closed loop formed by $\Cset$ and $\Saset{}$  when using \emph{unter-approximations} of $R$ and $T$. I.e., we replace $R$ and $T$ in \eqref{equ:Csetsound} by $\Rseta{l}\subseteq\Ya{l}$ and $\Tseta{l}\subseteq\Ya{l}$ for every \layer s.t.\ $\Rseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}}$ and $\Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset{}}$, respectively.
% % For \eqref{equ:Csetsound:safe}, that is, if $\xia(k)$ is a layer $l$ cell which is currently the largest cell in the domain of $\Cset$, then it must be contained in the under-approximation $\Rseta{l}$ of the safe set. 
% % Note that, in this case, the considered sampling instances might be non-uniformly spaced. 
% % This implies that we can find a 
% This ensures that a multi-layer controller $\Cset$ computed via $\Saset{}$ can be applied to the original control system $\Sigma$ in a sample-and-hold fashion to solve $\tuple{\Sigma,\Spec}$.
% 
% Obviously, the set $\WIN(\Sigma,\Spec)$ of controllers solving $\tuple{\Sigma,\Specs}$ is typically not a singleton; 

% \begin{remark}
%  It is common practice in ABCS to ensure safety for sampling times only. This implicitly assumes that sampling times and grid sizes are chosen such that no \enquote{holes} occur between consecutive cells visited in a trajectory. This can be formalized by additional assumptions on the growth rate of $f$ in \eqref{equ:def_f} which is beyond the scope of this paper.
% \end{remark}



% 
% $\Cset\in\WIN(\Sigma,\Spec)$ if for abstract trajectories 
% 
% To compute a multi-layered controller $\Cset\in\WIN(\Sigma,\Spec)$ with maximal domain, we want to utelize the constructed multi-layered abstraction $\Saset{}$. For this, we have to first \emph{unter-approximate} $R$ and $T$ by $\Rseta{l}\subseteq\Ya{l}$ and $\Tseta{l}\subseteq\Ya{l}$ for every \layer s.t.\ $\Rseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}}$ and $\Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset{}}$, respectively.
% \begin{equation}\label{equ:Csetsound}
%  \AllQ{\xia\in\Behaclset}{\AllQ{k\in\dom{\xia}}{\Qset^{-1}(\xia(k))\subseteq\Tset{}}}.
% \end{equation}
% 
% 
% When considering an 
% % 
% 
% 
% 
% 
% 
% 
% For a given layer $l\in [1;L]$, we define the over-approximation of the obstacles $O$ as
% %a (possibly empty) sub-cover $\Oa{}\subset\Ya{}$ over the set of obstacles states $O$ s.t.\ 
% \begin{equation}\label{equ:def:Oa}
%  \Oa{l} := \SetComp{\xa\in\Ya{l}}{\exists x\in \xa\;.\;x\in O},
% \end{equation}
% and the under-approximation of $\Tset{}$ w.r.t.\ $\Oa{l}$ as\footnote{
% 	We assume that all involved parameters and sets are such that $\Tseta{}\not=\emptyset$. 
% 	While this is not true in general, $T\not\subseteq O$ implies that there exists $\eta$ for which it is true.\label{fn_1}
% }
% \begin{align}\label{equ:ITseta}
%  \Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset\setminus \Oset}\setminus\Oa{l} \ .
% \end{align}


%Equivalently, there must exist a $k$ s.t.\ $\xia(k)$ is a layer $l$ cell which is currently the largest cell in the domain of $\Cset$ and is contained in the under-approximation $\Tseta{l}$ of the target set $\Tset$. 

% ************ Reduction of reach-avoid to reach via deletion of outgoing transitions from the obstacle states
%Now recall from \REFsec{sec:prelim} that the construction of $\Sa{}(\Sigma, \tau,\eta,\Spec) = (\Xa{},\Ua,\Fa{})$ ensures that 
%%every trajectory of the abstract closed loop remains within $Y$ and avoids $\Oa{}$. 
%whenever a trajectory exits the safe region $Y$ or enters an obstacle $O$ it gets blocked (since states in $(\Xa{}\setminus \Ya{})\cup \Oa{}$ don't have any outgoing transitions).
%Hence it is easy to see that one could reduce the original reach-avoid control problem to a simple reachability problem over the abstract state space.
%In other words, we say that $\Cset\in\WIN(\Sigma,\Spec)$ if for all $\xia\in\Behaclset$ it holds that
%\begin{align}\label{eq:sound abstract closed loop}
%%  \AllQ{\xia\in\Behaclset}{
% \propImp{
% \xia(0)\in\Uc
% }{
%\left( \exists k\in\dom{\xia}\;.\;\Qset^{-1}(\xia(k))\subseteq\Tset{}  \right)
% },
%%  },
%\end{align}
%and moreover $\dom{\Cset}$ is the largest possible.
%%To solve the reach-avoid control problem $\tuple{\Sigma,\Spec}$, it suffices to construct a multi-layered controller $\Cset$ solving the reachability control problem $\tuple{\Saset,\set{\Tseta{l}}_\layer}$ in the sense of \eqref{eq:sound abstract closed loop}, denoted by $\Cset\in\WIN(\Sigma,\Spec)$. 

% \smallskip
% \noindent\textbf{Safety Control Problem.}
% This problem was addressed in one of our previous papers \cite{hsu2018lazy}, and is summarized here for completeness.
% The safety specification is identified by the pair $\Specs = (Y, \Rset{})$ where $\Rset{}\subseteq \Xa{}$ is a set of safe states.
% %Consider a set of safe states $\Rset{}\subseteq Y\subseteq X$, where $Y$ is the global safety requirement used to construct the \emph{finite} abstractions $\set{\Sa{l}}_\layer$ (see \REFsec{sec:prelim}). 
% In LTL notation, the specification is given as 
% \begin{equation}
% 	\Specs = \text{always}\; (\Rset{}\cap Y).
% \end{equation}
% Like in reach-avoid, we keep the sets $Y$ and $\Rset{}$ separate in order to highlight the fact that $Y$ is embedded in the abstraction whereas $\Rset{}$ is dealt with in the synthesis stage.
% 
% We consider the safety control problem $\tuple{\Sigma,\Specs}$, which asks for a controller with maximal domain to be constructed such that every trajectory $\xi$ of the closed loop system stays within $\Rset{}\cap Y$ at \emph{sampling instances}.
% Formally, a multi-layered controller $\Cset$ therefore solves $\tuple{\Sigma,\Specs}$ if for all $\xit\in\Behtclset$ it holds that $\xit(k)\in\Rset{}\cap \Ya{}$ for all $k\in\dom{\xit}$. 
% Again, the considered sampling instances might be non-uniformly spaced.
% 



==> lazyReach.tex <==
%\begin{small}
\begin{algorithm}[t!]
	\caption{$\OTFAR_{m}$}\label{alg:OTFA subroutine}
	\begin{algorithmic}[1]
% 		\Require $T\subseteq \Xa{l}$, $\Aux\subseteq \Xa{1}$, $l$, $\Cset$
		\Require Winning domain $\Aux\subseteq \Xa{1}$, obstructions $\Oa{l}$, current layer $l$, set of controllers $\Cset$
		\If{$l=L$}
			\State $\langle W,C \rangle \gets \REACH_\infty(\UA{L1}(\Aux),\Oa{l},l)$   \label{alg:full reach}
			\State $\Cset \gets \Cset \cup \set{C}$ 	% For non-ranked set of controllers
			\State $\Aux \gets \Aux \cup \UA{1l}(W)$ // Save $W$ to $\Aux$ \label{alg:safe1}
%			\State $Push(\Cset,C)$	% For ranked set of controllers
			\If{$L=1$} \qquad // Single-layered reachability
				\State \Return $\langle \Aux,\Cset \rangle$ \label{alg:L=1}
			\Else \qquad // Go finer
% 				\State $W \gets \Gamma_{(l-1)l}(W) \cup \Gamma_{(l-1)1}(\Aux)$ \new{// Load $\Aux$} \label{alg:load1}
% 				 \State $\Aux \gets \Aux \cup \Gamma_{1l}(W)$ \new{// Save $W$ in $\Aux$} \label{alg:save1}
				\State \fbox{$\EXPLORE_m(\Aux,l-1)$}
				\State $\langle \Aux,\Cset \rangle \gets \OTFAR_{m}\left(\Aux,l-1,\Cset\right)$ \label{alg:go finer 1}
				\State \Return $\langle \Aux,\Cset \rangle$
			\EndIf
		\Else
			\State $\langle W,C \rangle \gets \REACH_m(\UA{l1}(\Aux),\Oa{l},l)$ \label{alg:compute reach}
			\State $\Cset \gets \Cset \cup \set{C}$ % For non-ranked set of controllers
			\State $\Aux \gets \Aux \cup \UA{1l}(W)$ // Save $W$ to $\Aux$ \label{alg:safe2}
%			\State $Push(\Cset,C)$	 % For ranked set of controllers
			\If{Fixed-point is reached in line \ref{alg:compute reach}} \label{alg:checkFP}
				\If{$l = 1$} // Finest layer reached \label{alg:terminate}
					\State \Return $\langle \Aux,\Cset \rangle$
				\Else \qquad // Go finer
					\State \fbox{$\EXPLORE_m(\Aux,l-1)$}
% 					\State $W \gets \Gamma_{(l-1)l}(W) \cup \Gamma_{(l-1)1}(\Aux)$ \new{// Load $\Aux$} \label{alg:load 2}
% 					\State $\Aux \gets \Aux \cup \Gamma_{1l}(W)$ \new{// Save $W$ in $\Aux$} \label{alg:save2}
					\State $\langle \Aux,\Cset \rangle \gets \OTFAR_{m}(\Aux,l-1,\Cset)$	\label{alg:go finer 2}
					\State \Return $\langle \Aux,\Cset \rangle$
				\EndIf
			\Else \qquad // Go coarser \label{alg:go coarser begin}
					\State \fbox{$\EXPLORE_m(\Aux,l+1)$}
% 				\State $\Aux \gets \Aux \cup \Gamma_{1l}(W)$ \new{// Save $W$ in $\Aux$} \label{alg:save3}
				\State $\langle \Aux,\Cset \rangle \gets \OTFAR_{m}(\Aux,l+1,\Cset)$	\label{alg:go coarser}
				\State \Return $\langle \Aux,\Cset \rangle$	\label{alg:go coarser end}
			\EndIf
		\EndIf
	\end{algorithmic}
\end{algorithm}
%\end{small}

\subsection{Synthesis Using Lazy Abstraction}\label{sec:LazyAbstraction}

%\section{Lazy Abstraction-Refinement}\label{sec:LazyAbstraction}
We now describe the main contribution of this paper, a lazy abstraction algorithm for reach-avoid specifications. The novelty with respect to the previous algorithm is encapsulated in the subroutine \REFalg{alg:EXPLORE subroutine}, whose usage in \REFalg{alg:OTFA subroutine} we previously ignored.

Let $\MLAR_{m}(\Tseta{1},\Oa{1},L)$ be a wrapper function which calls $\OTFAR_{m}$ in \REFalg{alg:OTFA subroutine} with arguments $(\Tseta{1},\Oa{1},L,\emptyset)$, but without assuming that $\Sa{l}$ is pre-computed for $l< L$. 
% Hence $\EXPLORE$ needs to be called within $\OTFAR_{m}$.
% Instead, the algorithm initially only computes $\Sa{L}$, the abstract system at the coarsest level $L$.
Hence, whenever the reachability algorithm at layer $l<L$ of $\OTFAR_{m}$ needs to access the abstract transition, the procedure $\EXPLORE_m$ is used to compute some of abstract transition function so that further progress in synthesis can be made.
% The soundness and completeness of $\MLAR_{m}$ follows from \REFthm{thm:EagerReach}, 
% if we can ensure that in every iteration of $\MLAR_{m}$ the set of states 
% returned by $\EXPLORE_m$, for which the abstract transition relation is computed, 
% is \emph{not smaller} than the set of states subsequently added to $\Aux$ by $\REACH_m$ in the next iteration. 
% % Being not smaller is important for completeness.


\begin{algorithm}[t]
	\caption{$\EXPLORE_m$ (for $\OTFAR$)}\label{alg:EXPLORE subroutine}
	\begin{algorithmic}[1]
		\Require Winning domain $\Aux\subseteq \Xa{1}$, current layer $l$
		\State $W' \gets \JUpre{l}^{m}(\OA{L1}(\Aux)) \setminus \UA{L1} (\Aux)$\label{alg:overapprox states} %. Both $\JUpre{\eta_{l_1}\tau_{l_2}}^{p}(\cdot)$ and $\OA{L1}(\cdot)$ potentially include some states occupied by obstacles in layer $L$. 
		% Version with general over approximation operator between any two layers 
%		\State $W' \gets \Upre_{p}(\Gamma_{L,1}^\uparrow(\Aux)) \setminus \Gamma_{L,1} (\Gamma_{L,1}^\uparrow(\Aux))$ where $Upre_{p}(\cdot)$ is the set of predecessor states in layer $L$ which are at most $p$ steps away, and $\Gamma_{l_2l_1}(\cdot)$ is the outer-approximation of a set of states in layer $l_1$ to layer $l_2$. Both $\Upre_{p}(\cdot)$ and $\Gamma_{l_2l_1}^\uparrow$ potentially include some states occupied by obstacles in layer $L$. \label{alg:overapprox states} \new{NEW} 
		\State $W'' \gets \UA{lL}(W')$ \label{alg:candidate states for explore}
		\State Compute $\Fa{l}$ as in \eqref{eq:next state abs sys 0} for all $\xa\in W''\setminus \Oseta{l}$ and $\tau=\tau_l$.\label{alg:partial abs}
	\end{algorithmic}
\end{algorithm}

\smallskip
\noindent\textbf{Constructing the Frontier.}
% 
$\EXPLORE_m$ determines which states it should compute transitions for by finding a set of \emph{frontier states} in the following manner: it computes the predecessors of the already-obtained set $\Aux$ optimistically by (i) using (coarse) auxiliary abstractions for this computation and (ii) applying a cooperative predecessor operator.

This requires a set of auxiliary systems, given by $\Aaset = \set{\Aa{l}}_{l=1}^L$, where $\Aa{l}:=\Sa{}(\Sigma,\tau_l,\eta_L) = (\Xa{L},\Ua,\Ja{l})$.
%Recall from \REFsec{sec:prelim} that this implies that $\Ja{l}$ is defined for all $\xa\in\Ya{L}$, $\xa'\in\Xa{L}$, and $u\in\Ua$ by \eqref{eq:next state abs sys 0} with $\tau=\tau_l$.
The abstract system $\Aa{l}$ induced by $\Sigma$ captures the $\tau_l$-duration transitions in the coarsest layer state space $\Xa{L}$.
Using $\tau_l$ instead of $\tau_L$ is important, as $\tau_L$ might cause \enquote{holes} between the computed frontier and the current target $\Upsilon$ which cannot be bridged by control actions in layer $l$.
This would render $\MLAR_{m}$ unsound.
%Ignoring $O$ is important, as usually $\Oa{l}\subset\Oa{L}$. 
Also note that in $\EXPLORE_m$, we ignore the obstacles altogether.
This is because $\Oa{l}\subseteq\Oa{L}$, and when the inequality is strict then the obstacle-free states in layer $l$ which are possibly winning but are covered by an obstacle in layer $L$ (see \REFfig{fig:informal example}) can also be explored.  

% KH: Was this the bug that you found, Kaushik? Haha.

For $\Aux\subseteq\Xa{L}$ and $l\in[1;L]$, we define the \emph{cooperative predecessor} operator
\begin{align}
\JUpre{l}(\Aux)= \set{\xa\in\Xa{L} \mid \exists \ua\in\Ua{}\;.\;\Ja{l}(\xa,\ua)\cap \Aux \neq \emptyset}. \label{eq:define upre}
\end{align}
Contrast this with the controllable predecessor operator~\eqref{eq:define cpre}.
We apply the cooperative predecessor operator $m$ times in $\EXPLORE_m$, i.e.,
% \begin{subequations}
\begin{align*}\label{eq:def upre^r}
&\JUpre{l}^1(\Aux)  = \JUpre{l}(\Aux)~\text{and}~\\ 
&\JUpre{l}^{j+1}(\Aux)  = \JUpre{l}^{j}(\Aux) \cup \JUpre{l}(\JUpre{l}^j(\Aux)). \numberthis
\end{align*}
% \end{subequations}

When calling $\EXPLORE_m$ with parameters $\Aux\subseteq \Xa{1}$ and $l<L$, it applies $\JUpre{l}^m$ to the over-approximation of $\Aux$ by abstract states in layer $L$. 
This over-approximation is defined as the dual operator of the under-approximation operator $\UA{ll'}$:
\begin{align}\label{eq:def over approx}
	\OA{ll'}(\Upsilon_{l'}) := \begin{cases}
								\Ra{ll'}(\Upsilon_{l'}), & l \leq l' \\
								\SetComp{\hat{x} \in \Xa{l}}{\Ra{l'l}(\hat{x})\cap \Upsilon_{l'} \neq \emptyset}, & l > l' 
							\end{cases}
\end{align}
where $l,l'\in [1;L]$ and $\Upsilon_{l'}\subseteq \Xa{l'}$. 
Finally, $m$ controls the size of the frontier set and determines the maximum progress that can be made in a single backwards synthesis run in a non-coarsest layer.

\smallskip
\noindent\textbf{Soundness and Relative Completeness.}
The soundness and relative completeness of $\MLAR_{m}$ follows from \REFthm{thm:EagerReach}, 
if we can ensure that in every iteration of $\MLAR_{m}$ the set of states 
returned by $\EXPLORE_m$, for which the abstract transition relation is computed, 
is \emph{not smaller} than the set of states subsequently added to $\Aux$ by $\REACH_m$ in the next iteration. 
% 
We obtain this result by the following series of lemmata, proven in the Appendix, leading to our main result stated in \REFthm{thm:LazyReach}. 

We first observe that computing the under-approximation of the $m$-step cooperative predecessor w.r.t.\ the auxiliary system $\Aa{l}$ of a set $\Aux_L$ (as used in $\EXPLORE_m$) over-approximates the set obtained by computing the $m$-step cooperative predecessor w.r.t.\ the abstract system $\Sa{l}$ for a set $\Aux_l$ (as used in $\REACH_m$) if $\Aux_L$ over-approximates $\Aux_l$. 

\begin{lemma}\label{lem:containment}
Let $\Saset$ be a multi-layered abstract system satisfying Assumption~\ref{assumption:monotonic approximation}, and let $\Aux_l\subseteq \Xa{l}$ and $\Aux_L\subseteq \Xa{L}$ for some $l<L$ s.t.\ $\Aux_L \supseteq \OA{Ll}(\Aux_l)$. Then $\UA{lL}(\JUpre{l}(\Aux_L)) \supseteq \FUpre{l}(\Aux_l)$. Furthermore, for all $m>0$, it holds that $\UA{lL}(\JUpre{l}^m(\Aux_L)) \supseteq \FUpre{l}^m(\Aux_l)$, where $\FUpre{l}$ and $\FUpre{l}^m$ for $\Sa{l}$ are defined analogously to \eqref{eq:define upre} and \eqref{eq:def upre^r}, respectively.
\end{lemma}

\REFlem{lem:containment} can be used to show that $\EXPLORE_m$ constructs the transition function $\Fa{l}(\xa,\ua)$ for all $\xa$ which are in the winning state set computed by $\REACH_m$.

\begin{lemma}\label{lem:single iteration}
%  Let $P$ denote the number of recursive calls of $\OTFAR_{m,r}$ needed in $\MLAR_{m,r}$ before $\OTFAR_{m,r}$ terminates, i.e., line~\ref{alg:terminate} becomes true. Suppose that for iteration $p\in[1;P]$ the algorithm $\OTFAR_{m,r}$ is called with $\Aux\in\Xl{1}$ and $l=\lp<L$, and hence line~\ref{alg:terminate} executes returning the controller $\Ci{p}=(\Uci{p},\Ua,\Gci{p})$. 
For all $l<L$, $\Aux\subseteq\Xa{1}$ and $C=(\Uci{},\Ua,\Gci{})$ returned by $\REACH_m(\UA{l1}(\Aux),\Oa{l},l)$, it holds that $\xa\in\Uci{}\setminus \UA{l1}(\Aux)$ implies $\xa\in W''$, where $W''$ is returned by the second line of $\EXPLORE_m(\Aux,l)$.
\end{lemma}

With \REFlem{lem:single iteration}, soundness and relative completeness of $\MLAR_{m}$ directly follows from \REFthm{thm:EagerReach}, as proven in the Appendix.

\begin{theorem}\label{thm:LazyReach}
Let $\tuple{\Sigma,\Specr}$ be a reach-avoid control problem and $\Saset = \set{\Sa{l}}_\layer$ a sequence of abstractions. 
Let $\langle \Aux^N,\Cset \rangle=\mathsf{LazyReach}_m(\Tseta{1},\Oa{1},L)$. 
Further, let $C = (B,\Ua{},G)$ be returned by $\REACH_\infty(\Tseta{1},\Oa{1},1)$.
Then $\Cset$ is sound and relatively complete, in the sense of the statement of \REFthm{thm:EagerReach}, w.r.t.\ single-layer control for layer $l=1$. 
\end{theorem}

% \begin{theorem}\label{thm:sound and complete MLAR}
% The multi-layered controller $\Cset$ computed by $\MLAR_{m}$ is composable with $\Saset$ and the behaviour $\Behaclset$ of the closed loop formed by $\Saset$ and $\Cset$ satisfies
% \eqref{eq:sound abstract multi-layered closed loop}, 
% % for all $\xia\in\Beh{\Sa{}^{cl}}$ with $\xia(0)\in\Iseta{}$ exists some $k\in\dom{\xia}$ s.t.\ $\xia(k)\in\Tseta{}$
% % \begin{align}\label{eq:sound abstract multi-layered closed loop}
% %  \AllQ{\xia\in\Behaclset}{
% %  \propImp*{
% %  \xia(0)\in\dom{\Cset}
% %  }{
% %  \ExQ*{k\in\dom{\xia}}{\Qa{1}\left(\Qset^{-1}(\xia(k))\right)\in\Tseta{1}}
% %  }
% %  }.
% % \end{align}
% i.e., $\Cset$ is a sound.
% Furthermore, let $C = (B,\Ua{},G)$ be returned by $\REACH_\infty(\Tseta{1})$, i.e.\ $\C\in\WIN(\Sa{1},\Tseta{1})$. Then $\Qa{1}\left(\Qset^{-1}(\dom{\Cset})\right)= B$, i.e. $\Cset$ is complete. 
% \end{theorem}






==> lazySafe.tex <==
\subsection{Synthesis Using Lazy Abstraction}\label{sec:ML_Safety_Frontier}

We now consider the case where the multi-layered abstraction $\Saset$ is not pre-computed. This is implemented by a wrapper function $\MLASAFE(\Rseta{1},L)$ which simply calls $\OTFAS{}(\Rseta{1},\emptyset,L,\emptyset)$. % and returns the computed value.
% \begin{algorithm}[]
% 	\caption{Procedure $\textproc{LazySafe}$}\label{alg:LazySafe}
% 	\begin{algorithmic}[1]
% 		\Require $\Aux\subseteq \Xa{1}$, $L$
% % 		\State $\textproc{Explore}(\UA{l1}(\Aux),L)$
% % 		\For {$\layer$}
% % 		    \State $\textproc{Explore}^L_l(\OA{L1}(\Aux),l)$\label{alg:EagerSafe:computeAa}
% % 		\EndFor
% %                 \State $\Aux\gets \textproc{SafeIt}(\Aux,\emptyset,L,\emptyset)$
% %                 \State \Return $\Aux$
% 		\State \Return $\textproc{SafeIt}(\Aux,\emptyset,L,\emptyset)$
% 	\end{algorithmic}
% \end{algorithm}
% 
With this, Line~\ref{alg:SafeIt:Explore} of \REFalg{alg:SafeIt} is used to explore transitions in all states in layer $l$ which are (i) not marked unsafe by all layers in the previous iteration, i.e., are in $\UA{l1}(\Aux)$, but (ii) cannot stay safe for $i$ time-steps in any layer $l'>l$, i.e., are not in $\UA{l1}(\Aux')$. 
%  
In the first iteration of $\OTFAS{}(\Rseta{1},\emptyset,L,\emptyset)$ the set $\UA{l1}(\Aux)\setminus\UA{l1}(\Aux')$ is same as $\UA{1L}(\Rseta{1})=\Rseta{L}$. Hence, for layer $L$ all transitions for states inside the safe set are pre-computed in the first iteration of \REFalg{alg:SafeIt}. % and $\textproc{Explore}$ does not perform any computations for layer $L$ in further iterations. 
This is in general not true for lower layers $l<L$. %, as $\UA{1l}(\Aux')$ does usually not stay empty.

To ensure that the lazy exploration of the state space is still sound and relatively complete, we show in the following lemma that all states which need to be checked for safety in layer $l$ of iteration $i$ are indeed explored.

% % \smallskip
% % \noindent\textbf{Soundness and Relative Completeness}
% It is easy to see that soundness and relative completeness of $\textproc{LazySafe}$ directly follows from \REFthm{thm:EagerSafe} if for every layer $l$ and iteration $i$ of $\textproc{SafeIt}$ we have that the set of states explored in Line~\ref{alg:SafeIt:Explore} of \REFalg{alg:SafeIt} is larger then the set $\UA{1l}(W)\setminus\Aux'$ if $W$ would have been computed using the full transition system $\Sa{l}$ when evaluating Line~\ref{alg:SafeIt:computeW} of \REFalg{alg:SafeIt}. This follows from the ranking argument over $\Aux$ used in the proof of \REFthm{thm:EagerSafe} as formalized  the following lemma.

\begin{lemma}\label{lem:EffectLazyness}
%  Let $\Aux^i$ be defined as in \REFlem{lem:monotonicity} and define $\widetilde{\Aux}^i$ analogously for a call of $\textproc{SafeIt}$ by $\textproc{LazySafe}(\Rseta{1},L)$. Then it holds for all $i$ that $\Aux^i=\widetilde{\Aux}^i$.
Let $W^i_l$ and $\Aux'^i_l$ (resp. $\widetilde{W}^i_l$ and $\widetilde{\Aux}'^i_l$) denote the set computed in Lines~\ref{alg:SafeIt:computeW} and \ref{alg:SafeIt:safeW} of \REFalg{alg:SafeIt} (called by $\MLSAFE{}(\Rseta{1},L)$ and $\MLASAFE{}(\Rseta{1},L)$, resp.) the $i$-th time for layer $l$.  
% Let furthermore $\Aux'^i_{L+1}=\widetilde{\Aux}'^i_{L+1}=\emptyset$. \KM{I don't think this is needed, as one of the reviewers also thinks.}
Then it holds for all $i\in [1;N]$ and \layer that
 \begin{align}\label{equ:tildeWpl}
  %W^i_l\setminus\UA{l1}(\Aux'^i_{l-1})\subseteq
  \widetilde{W}^i_l\subseteq W^i_l\quad\text{and}\quad \Aux'^i_{l}=\widetilde{\Aux}'^i_{l}.
 \end{align}
\end{lemma}

Now as direct consequence of \REFthm{thm:EagerSafe} and \REFlem{lem:EffectLazyness}, we obtain:

%With this, we can show our second main result, namely that $\textproc{LazySafe}(\Rseta{1},L)$ is sound and relatively complete, which is a direct consequence of \REFthm{thm:EagerSafe} and \REFlem{lem:EffectLazyness}.

\begin{theorem}\label{thm:LazySafe}
Let $\tuple{\Sigma,\Specs}$ be a safety control problem and $\Saset = \set{\Sa{l}}_\layer$ a sequence of abstractions. Let $\langle \Aux^N,\Cset \rangle=\MLASAFE{}(\Rseta{1},L)$ s.t.\ $\Cset=\set{\Ci{l}}_\layer$ and $\Gci{l}$ be defined as in \eqref{def:safecontrollerGci} for all \layer.
Further, let $\overline{B}$ be the domain of the single-layer safety controller computed using \eqref{equ:safe-fp} for $l=1$.
Then $\Cset\in\WIN(\Sigma,\Specs)$ and $\overline{B}\subseteq\Aux^N$, i.e., $\Cset$ is sound and relatively complete w.r.t.\ single-layer control for layer $l=1$. 
\end{theorem}





% \smallskip
% \noindent\textbf{Auxiliary Systems}
% The set of auxiliary systems is given by $\Aaset = \set{\Aa{l}}_{l=1}^L$, where $\Aa{l}:=\Sa{}(\Sigma,\tau_l,\eta_L) = (\Xa{L},\Ua,\Ja{l})$.
% Recall from \REFsec{sec:prelim} that this implies that $\Ja{l}$ is defined for all $\xa\in\Ya{L}$, $\xa'\in\Xa{L}$, and $u\in\Ua$ by \eqref{eq:next state abs sys 0} with $\tau=\tau_l$.  Intuitively, $\Aa{l}$ is the abstract system induced by $\Sigma$, whose transition system indicates which layer $L$ cells are reachable from other layer $L$ cells by applying a constant control input for duration $\tau_l$, $l\leq L$. Using $\tau_l$ instead of $\tau_L$ is important, as $\tau_L$ might cause \enquote{holes} between the computed frontier and the safe set which cannot be bridged by control actions in layer $l$. 
% 
% For $\Aux\subseteq\Xa{L}$ and $l\in[1;L]$, we define the co-operative predecessor operator
% \begin{align}
% \JUpre{l}(\Aux)= \set{\xa\in\Xa{L} \mid \exists \ua\in\Ua{}\;.\;\Ja{l}(\xa,\ua)\cap \Aux \neq \emptyset} \label{eq:define upre}
% \end{align}
% and the over-approximation of states sets as
% \begin{align}\label{eq:def over approx}
% 	\OA{ll'}(\Upsilon_{l'}) := \begin{cases}
% 								\Ra{ll'}(\Upsilon_{l'}), & l \leq l' \\
% 								\SetComp{\hat{x} \in \Xa{l}}{\Ra{l'l}(\hat{x})\cap \Upsilon_{l'} \neq \emptyset}, & l > l' 
% 							\end{cases}
% \end{align}
% where $l,l'\in [1;L]$ and $\Upsilon_{l'}\subseteq \Xa{l'}$. 
% 
% 
% \smallskip
% \noindent\textbf{Partial Local Exploration} The basic idea of the frontier computation from \cite{} is to pre-compute all auxiliary transition systems $\Aaset$ in the wrapper function, now called $\textproc{LazySafeFrontier}$ (see \REFalg{alg:EagerSafe}) and to only explore those states in layer $l$ and iteration $i$ of \REFalg{alg:SafeIt} which are contained in the cooperative predecessor of the current safe set, evaluated using the auxiliary system $\Aa{l}$. 
% 
% This is formalized by the new wrapper function $\textproc{LazySafeFrontier}$ given in \REFalg{alg:EagerSafe}, which is essentially equivalent to $\textproc{EagerSafe}$, with the only difference that it now pre-computes $\Aaset$ instead of $\Saset$, which is substantially more efficient as it uses a large grid size only. The procedure $\textproc{Explore}^L_l$ called in Line~\ref{alg:EagerSafe:computeAa} of \REFalg{alg:EagerSafe} is equivalent to \REFalg{alg:Explore} except for computing $\Ja{l}$ instead of $\Fa{l}$.
% % 
% \begin{algorithm}[]
% 	\caption{Procedure $\textproc{LazySafeFrontier}$}\label{alg:LazySafeFrontier}
% 	\begin{algorithmic}[1]
% 		\Require $\Aux\subseteq \Xa{1}$, $L$
% 		\State $\textproc{Explore}(\UA{l1}(\Aux),L)$
% 		\For {$\layer$}
% 		    \State $\textproc{Explore}^L_l(\OA{L1}(\Aux),l)$\label{alg:EagerSafe:computeAa}
% 		\EndFor
%                 \State $\Aux\gets \textproc{SafeIt}(\Aux,\emptyset,L,\emptyset)$
%                 \State \Return $\Aux$
% 	\end{algorithmic}
% \end{algorithm}
% % 
% \begin{algorithm}[]
% 	\caption{Procedure $\textproc{Frontier}$}\label{alg:Frontier}
% 	\begin{algorithmic}[1]
% 	 \Require $\Aux\subseteq \Xa{1}$, $\Aux'\subseteq \Xa{1}$, $l$
% % 	      \State $\da{l}^L\gets\textproc{Explore}_\infty(\OA{L1}(\Aux),\da{l}^L,l)$
% 	      \State $\Aux''\gets\textproc{CoopSafe}(\OA{L1}(\Aux),l)$\label{alg:Frontier:CoopSafe}
% 	      \State \Return $\UA{lL}(\Aux'')\setminus\UA{l1}(\Aux')$
% 	\end{algorithmic}
% \end{algorithm}
% % 
% The outlined frontier computation is formalized by $\textproc{Frontier}$ (see \REFalg{alg:Frontier}). The procedure $\textproc{CoopSafe}$ called in Line~\ref{alg:Frontier:CoopSafe} of \REFalg{alg:Frontier} is equivalent to $\textproc{CSafe}$ when replacing Line~\ref{alg:CSafem:Iteration} in \REFalg{alg:CSafem} with the cooperative safety-iteration
% $\Aux' \gets \JUpre{l}(\Aux) \cap \Aux$.
% 
% It is easy to see that $\Aa{L}=\Sa{L}$. With this, we see that the pre-computation of $\Aa{L}$ implies that no frontier computation and exploration is necessary for layer $L$. In our implementation of $\textproc{LazySafeFrontier}$ we therefore omit Line~\ref{alg:SafeIt:Explore} of \REFalg{alg:SafeIt} whenever $l=L$. This does obviously not change the algorithm.
% 
% Of cause, pre-computing all auxiliary systems $\Aaset$ and evaluating the cooperative predecessor in every step causes a computational overhead compared to $\textproc{LazySafe}$. However, as we will show in \REFsec{}, this overhead is very small due to the large grid size used for its computation. Therefore, we still observe computational savings for particular examples using $\textproc{LazySafeFrontier}$ compared to $\textproc{LazySafe}$.
% % 
% \AKS{This is what I really would like to see empirically! Also the effect of $m$. Both effects might be correlated!}




==> reach.tex <==
\section{Abstract Reach-Avoid Control}
\label{sec:reach-avoid-control}

We propose to use multi-layered abstraction to solve the reach-avoid controller synthesis problem.
First, let us define approximations of the target and the obstacle sets using the abstract states.
For a given layer $l\in [1;L]$, we define the over-approximation of the obstacles $O$ as
%a (possibly empty) sub-cover $\Oa{}\subset\Ya{}$ over the set of obstacles states $O$ s.t.\ 
\begin{equation}\label{equ:def:Oa}
 \Oa{l} := \SetComp{\xa\in\Ya{l}}{\exists x\in \xa\;.\;x\in O},
\end{equation}
and the under-approximation of $\Tset{}$ w.r.t.\ $\Oa{l}$ as\footnote{
	We assume that all involved parameters and sets are such that $\Tseta{}\not=\emptyset$. 
	While this is not true in general, $T\not\subseteq O$ implies that there exists $\eta$ for which it is true.\label{fn_1}
}
\begin{align}\label{equ:ITseta}
 \Tseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Tset\setminus \Oset}\setminus\Oa{l} \ .
\end{align}

\sloppy By adopting the classical result of ABCS using FRR (see \cite[Sec.VI.A]{ReissigWeberRungger_2017_FRR}) to the multi-layered case (see \cite{hsu2018multi}, Sec.~3.4), we know that a multi-layered controller $\Cset$ enforces $\tuple{\Sigma,\Specr}$ if it solves the corresponding reach-avoid control problem on the multi-layered abstract system $\Saset$ for the target states $\set{\Tseta{l}}_{l\in [1;L]}$ and the obstacles $\set{\Oa{l}}_{l\in [1;L]}$.
In other words, $\Cset\in\WIN(\Sigma,\Specr)$ if for all $\xia\in\Behaclset$ it holds that
% for abstract trajectories of the closed loop formed by $\Cset$ and $\Saset{}$ holds that
$
%  \AllQ{\xia\in \dom{\Cset}}{
 \propImp{
 \xia(0)\in\Uc
 }{
\left( \exists k\in\dom{\xia}\;.\;\Qset^{-1}(\xia(k))\subseteq\Tset{}  \wedge \forall 1\leq k'\leq k\;.\;\Qset^{-1}(\xia(k'))\subseteq Y\setminus O\right)
 },
%  },
$
and moreover $\dom{\Cset}$ is the largest possible.

\subsection{Synthesis Using Exhaustive Abstraction.}

We now define the \emph{controllable predecessor} operator $\FCpre{l}:\twoup{\Xa{l}}\fun\twoup{\Xa{l}}$, which is a key component of all synthesis procedures to be presented:
\begin{equation}
 \FCpre{l}\left(\Aux\right) = \set{\xa\in\Xa{l} \mid \exists \ua\in\Ua{}\;.\;\Fa{l}(\xa,\ua) \subseteq \Aux}. \label{eq:define cpre}\\
\end{equation}

\smallskip
\noindent\textbf{Single-Layered Control.}
We recall how the reach-avoid control problem is commonly solved by a single-layered abstract system $\Sa{l}$ for the target $\Tseta{l}$ and the obstacle $\Oa{l}$.
% 
In this case one iteratively computes
\begin{equation}\label{equ:reach-fp}
	W^0 = \Tseta{l} \text{ and } W^{i+1} = \left(\FCpre{l}(W^i)\setminus \Oa{l}\right) \cup \Tseta{l}
\end{equation}
until some iteration $N\in \mathbb{N}$ is reached where $W^N = W^{N+1}$. 
The controller $C = (B,\Ua{},G)$ with $B = W^N\setminus \Tseta{}$ and
\begin{equation}\label{equ:reach-controller}
	G(\xa) = \set{\ua\in \Ua{} \mid \Fa{l}(\xa,\ua) \subseteq W^{i*}}
\end{equation}
for all $\xa\in B$, where $i^* = \min(\set{i \mid \xa\in W^i\setminus \Tseta{}})- 1$, is known to be a reachability controller for $\Tseta{l}$ \cite{MPS95}. 
Note that the ``avoid $\Oa{l}$'' part of the specification is taken care of by ignoring the states in $\Oa{l}$ which contribute to the $\FCpre{l}$ computation in the iteration \eqref{equ:reach-fp}. 
\KM{The reference is for reachability. Is there a reference for reach-avoid that uses this fixpoint?}
%\KM{Added the -1 (highlighted). Please check. If $\xa$ is itself in $i$, then it has to go one level down.}

We denote the procedure implementing this iterative computation until convergence $\REACH_\infty(\Tseta{l},\Oa{l},l)$.
% The controller returned by $\REACH_\infty(\Tseta{l},l)$ is sound, i.e., the abstract closed loop $\Behacl{l}$ satisfies 
% \eqref{eq:sound abstract closed loop}. % for $\Iseta{}=\Uc{}$. 
%Additionally, we have that $\C\in\WIN(\Sa{},\Iseta{},\Tseta{})$ if $\Iseta{} \subseteq B$.
% 
We shall also use a version of $\REACH$ which runs $m>0$ steps of \eqref{equ:reach-fp}.
Formally, the algorithm $\REACH_m(\Tseta{l},\Oa{l},l)$ returns the set $W^m$ (the result of the $m$-th iteration of \eqref{equ:reach-fp})
and the corresponding controller $C$ computed using $W^m$ in \eqref{equ:reach-controller}.
Note that if the iteration in \eqref{equ:reach-fp} reaches a fixed point in at most $m$ iterations,
$\REACH_\infty$ and $\REACH_m$ return the same result.


\smallskip
\noindent\textbf{Multi-Layered Control.}
We now recall the synthesis of a multi-layered controller $\Cset$ for the reach-avoid specification $(Y,T,O)$ using the multi-layered abstraction $\Saset$ \cite{hsu2018multi}. %the abstract reachability control problem $\tuple{\Saset,\set{\Tseta{l}}_\layer}$ presented in \cite{hsu2018multi}.
% 
This algorithm is given by a wrapper function $\mathsf{EagerReach}_m(\Tseta{1},\Oa{1},L)$, which calls the iterative algorithm $\OTFAR_{m}$ in \REFalg{alg:OTFA subroutine} with parameters $(\Tseta{1},\Oa{1}, L, \emptyset)$ under the assumption that $\Saset$ is pre-computed for all $\layer$ and $\EXPLORE_m$ is never called (i.e., the boxed lines of \REFalg{alg:OTFA subroutine} are ignored for this section).

The recursive procedure $\OTFAR_m$ in \REFalg{alg:OTFA subroutine} essentially implements the flow-chart of \REFfig{fig:flowchart} by ignoring the green box, which corresponds to the subroutine $\EXPLORE_m$ discussed in \REFsec{sec:LazyAbstraction}.
Lines 1--11 implement reach-avoid at the coarsest layer $\Sa{L}$, followed by $\OTFAR_m$ recursively calling itself to see if the winning states can be extended by a lower abstraction layer.
Lines 12--29 implement reach-avoid in a lower layer $(l < L)$, where the analysis is performed only for $m$ steps for a given fixed parameter $m>0$.
If the analysis already reaches a fixed point, then, as in the first case, the algorithm checks if further
states can be added in a lower layer (lines 16--23).
If not, the algorithm attempts to take the new states found by the reachability analysis, compute
an under-approximation in a coarser layer, and recursively continues the search at the coarser layer (lines 24--28).

In order to map abstract states between different layers of abstraction, we use the operator 
	\begin{equation}\label{equ:Gamma}
	 		\UA{ll'}(\Upsilon_{l'}) = 
			\begin{cases}
				\Ra{ll'}(\Upsilon_{l'}), & l \leq l' \\
				\SetComp{\hat{x} \in \Xa{l}}{\Ra{l'l}(\hat{x})\subseteq \Upsilon_{l'}}, & l > l' 
			\end{cases}
	\end{equation}
where $l,l'\in [1;L]$ and $\Upsilon_{l'}\subseteq \Xa{l'}$. 
The operation $\UA{ll'}(\Upsilon_{l'}) \subseteq \Xa{l}$ under-approximates a set $\Upsilon_{l'} \subseteq \Xa{l'}$
with one in layer $l$. 

It is proven in \cite{hsu2018multi} that $\mathsf{EagerReach}_m$ is sound and relatively complete w.r.t.\ single-layered control using the finest layer $l=1$.

\begin{theorem}[\cite{hsu2018multi}]\label{thm:EagerReach}
Let $\tuple{\Sigma,\Specr}$ be a reach-avoid control problem and $\Saset = \set{\Sa{l}}_\layer$ a sequence of abstractions. 
Let $\langle \Aux^N,\Cset \rangle=\mathsf{EagerReach}_m(\Tseta{1},\Oa{1},L)$. 
Further, let $C = (B,\Ua{},G)$ be returned by $\REACH_\infty(\Tseta{1},\Oa{1},1)$.
Then 
\begin{inparaenum}[(a)]
	\item $\Cset\in\WIN(\Sigma,\Specr)$: referred to as $\Cset$ being sound, and 
	\item $\overline{B}\subseteq\Aux^N$: referred to as $\Cset$ being relatively complete w.r.t.\ single-layered control for layer $l=1$. 
\end{inparaenum}
\end{theorem}

% \begin{theorem}[\cite{HsuMajumdarMallikSchmuck_HSCC18}]\label{thm:reach is sound and complete}
% Let $\Sigma$ be a control system, $\Spec = \braket{Y}{T}{O}$ a specification
% % Let $\n{1}>0$, $\ta{1}>0$, and for $l\in[2;L]$, let $\n{l} = 2 \n{l-1}$ and $\ta{l} = 2\ta{l-1}$.
% and $\Saset = \set{\Sa{l}(\Sigma,\ta{l},\n{l},\Spec)}_\layer$ a sequence of abstractions.
% For every $m>0$, if $\mathsf{EagerReach}_m(\Tseta{1}, L, \emptyset)$ returns $\Aux \subseteq \Xa{1}$ and 
% a multi-layered controller $\Cset$,
% then $\Cset$ is composable with $\Saset$ and the behavior $\Behaclset$ of the closed loop of $\Saset$ and $\Cset$ satisfies 
% % for all $\xia\in\Beh{\Sa{}^{cl}}$ with $\xia(0)\in\Iseta{}$ exists some $k\in\dom{\xia}$ s.t.\ $\xia(k)\in\Tseta{}$
% \begin{multline}\label{eq:sound abstract multi-layered closed loop}
%  \forall\xia\in\Behaclset \; . \; 
%  \left(
%  \xia(0)\in\dom{\Cset} \Rightarrow \right.\\
%  \left.\left( \exists k\in\dom{\xia} \; . \; \Qa{1}\left(\Qset^{-1}(\xia(k))\right)\in\Tseta{1} \right)\right),
% \end{multline}
% i.e., $\Cset$ is sound.
% Furthermore, let $C = (B,\Ua{},G)$ be returned by $\REACH_\infty(\Tseta{1})$, i.e.\ $\C\in\WIN(\Sa{1},\Tseta{1})$. Then $\Qa{1}\left(\Qset^{-1}(\dom{\Cset})\right)= B$, i.e. $\Cset$ is complete. 
% % \KM{Need to be careful with $\Behaclset$, because at every sampling the state belongs to a different abstraction. I think we should explicitly define this in Section 2.}
% \end{theorem}


\input{lazyReach}


==> related.tex <==

\section{Related Work}
This work is based on our multi-layered ABCS technique introduced in \cite{hsu2018multi} and an extension to lazy abstraction for safety specifications in \cite{hsu2018lazy}. The present paper extends \cite{hsu2018multi} to lazy abstraction for reach-avoid specifications instead. To handle this specification class, we introduce auxiliary abstract systems in order to enable local exploration of the transition system, which was not required in \cite{hsu2018lazy}. %\TODO{How is this different from the exploration in \cite{nilsson2017augmented, bulancea2018nonuniform}?}

The idea of using multiple abstractions of varying granularity in the context of controller synthesis is not new. 
However, most prior works assume \emph{linear} dynamical systems \cite{aydin2012language,girard2006towards} which allows for the use of polytopic approximations, assume \emph{unperturbed} systems \cite{aydin2012language,rungger2012fly,grune1997adaptive,pola2012integrated,CameraGirardGoessler_reach_2011,Girard2016_InterSampling} which allows for very efficient forward search-based synthesis techniques, or assume that the system dynamics are \emph{stable} in some sense \cite{Girard2016_InterSampling,CameraGirardGoessler_safety_2011,CameraGirardGoessler_reach_2011}.
The method presented in \cite{CameraGirardGoessler_reach_2011,Girard2016_InterSampling} is implemented in the tool CoSyMA \cite{mouelhi2013cosyma} which enjoys these benefits. 
However, our implementation in MASCOT (also applicable to perturbed systems) still slightly outperforms CoSyMA on an unperturbed dc-to-dc boost converter example\footnote{This experiment was performed with a 2.7 GHz Intel Core i5 processor and 16 GB memory. Details can be found in the MASCOT repository.} (205 s versus 235 s). 

% When it comes to similar techniques for perturbed non-linear systems, the literature is rather sparse.
% For \emph{perturbed non-linear systems}, there exists approach by
% Fribourg et al.\ 
% % propose a technique for perturbed polynomial systems 
% % that 
% which relies on successive decomposition \cite{fribourg2013constructing} 
For \emph{perturbed nonlinear systems}, there exists a successive decomposition approach \cite{fribourg2013constructing,fribourg2014finite} which is restricted to polynomial and affine dynamics, respectively.
% \KH{the extension seems to have been published before the original?}. 
This method heavily relies on an ad-hoc computation of a linear over-approximation of the given polynomial system, which hinders automation of the ABCS work-flow.

Recently, Nilsson et al. presented an abstraction-refinement technique for perturbed nonlinear systems \cite{nilsson2017augmented,bulancea2018nonuniform}, which shares with our approach the idea of using particular candidate states for \emph{local} refinement. However, the works differ by the way abstractions are constructed.
The approach in \cite{nilsson2017augmented} identifies all adjacent cells which are reachable using a particular input, splitting these cells for finer abstraction computation. This is analogous to established abstraction-refinement techniques for solving two-player games \cite{AlfaroRoy_2010}. On the other hand, our method computes reachable sets for particular sampling times that vary across layers, resulting in a more delicate abstraction-refinement loop. Our approach also handles more general dynamics and establishes feedback-refinement relations, which are advantageous for controller design (see \cite{ReissigWeberRungger_2017_FRR} for an in-depth discussion).
%\footnote{Our attempt to provide a quantitative comparison of MASCOT with the tool ARCS implementing the approach in \cite{nilsson2017augmented,bulancea2018nonuniform} failed as the latter tool currently does not support obstacles in the state space which is essential to see a benefit of a multi-layered approach.}.

The lazy ABCS for safety specification appeared in an earlier paper \cite{hsu2018lazy}, and a summary of the respective related work can be found there.

% ************* safety related work (needed?) *****************
%The safety part is an improvement over \cite{hsu2018multi} by means of a novel fix-point. 
%In \cite{hsu2018multi}, starting from the coarsest layer a reach-or-stay control problem is solved successively till the finest layer is reached.
%In each layer, the target set for the reachability objective is the winning set from the immediate coarser layer, and the safe set for the safety objective is the inner-approximation of the given safe set.
%This might result in an undesirable situation when the finer layers are used unnecessarily more often than the coarser layers \cite{hsu2018lazy}.
%This situation is avoided in our new algorithm, which runs 2x faster than the one presented in \cite{hsu2018multi} on a particular example.
%
%The multi-layered ABCS algorithm for safety specifications by Girard et al. \cite{Girard2016_InterSampling} considers a strict subclass of 
%the dynamics considered in this paper and uses a modified version of approximate bisimulation relations instead of the more general FRR considered in this paper. This results in a deterministic abstract model, which allows for a forward search based technique to synthesize safety controllers. 
%While forward search is usually faster for safety, it is not known how to symbolically handle external disturbances and non-determinism 
%in the abstraction in a forward algorithm.%, and 
%%how controllers for $\omega$-regular objectives can be computed over the resulting non-deterministic game graphs efficiently.
%
%% \new{
%Meyer et al. propose an abstraction refinement algorithm for a fragment of LTL specifications \cite{meyer2017abstraction}, where a nominal single integrator model is used to find a viable plan which is used to refine abstractions locally along the planned path. As the nominal model is not based on the system dynamics, this heuristic may or may not give quick convergence. Our approach does not suffer from this problem.
%
%Nilsson et al. propose an abstraction refinement technique to synthesize switching protocols for switched systems and reach-avoid-stay specifications \cite{nilsson2014incremental}. The ``stay'' part of their algorithm solves a safety game while adaptively refining the abstraction as needed. This algorithm suffers from the same problem as \cite{hsu2018multi}.
% ************* upto here: this is a copy of the cdc paper's related work

% \TODO{Finish}\KM{This is the trickiest comparison. Note that the reviewers did not suggest a comparison with these papers, but I think these two are the closest related papers. I do not see any shortcoming of \cite{nilsson2017augmented,bulancea2018nonuniform} compared to our paper. The only hope was that our implementation is faster. I was playing with the example that they use in their paper for comparison. For that example, our implementation is slower. My hope is that our algorithm will have an upper hand for fast dynamics. But I need to run more experiments before I can say something conclusive.}
% 
 
% 
% If we move away from the setting of continuous dynamical systems, and instead consider more abstract setting of two-player graph games, our algorithm bears some similarity to the three-valued abstraction-refinement scheme proposed by Alfaro et al.\ \cite{AlfaroRoy_2010}. However, due to the use of different sampling times in different abstraction layers in our setting---which is unavoidable in the context of dynamical systems---we cannot apply their method to determine an exact frontier. %Instead, we use the tuning parameter $m$ to bound the number of calls to the fixed-point algorithm in every iteration to balance the over-approximation of the frontier. 



==> safe.tex <==
\section{Abstract Safety Control \cite{hsu2018lazy}}

This section builds towards and presents the multi-layered controller synthesis procedure for safety specifications introduced in \cite{hsu2018lazy}.
All proofs are omitted due to space constraints, and can be found in the original paper \cite{hsu2018lazy}.

We recall that (see \cite{hsu2018multi}, Sec.~3.4) if for the abstract trajectories of the closed loop formed by $\Cset$ and $\Saset{}$ the following holds:
\begin{equation}\label{equ:Csetsound}
 \AllQ{\xia\in\Behaclset}{\AllQ{k\in\dom{\xia}}{\Qset^{-1}(\xia(k))\subseteq\Rset{}\cap Y}},
\end{equation}
then the refinement of $\Cset$ fulfills $(\Sigma,\Specs)$.
In this regard, we define an under-approximation of the safe set $\Rset{}$ in each abstraction layer as $\Rseta{l}:=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}} \subseteq\Ya{l}$.
%
%When considering an under-approximation of $\Rset{}$ by $\Rseta{l}\subseteq\Ya{l}$ for every \layer s.t.\ $\Rseta{l}=\SetComp{\xa\in\Xa{l}}{\xa\subseteq \Rset{}}$, the right side of \eqref{equ:Csetsound} states that $\xia(k)\in\img{\Qset}\cap\Xa{l}$ implies $\xia(k)\in\Rseta{l}$. That is, if $\xia(k)$ is a layer $l$ cell which is currently the largest cell in the domain of $\Cset$, then it must be contained in the under-approximation $\Rseta{l}$ of the safe set. 
%% 
We collect all multi-layered controllers which solve $\tuple{\Sigma,\Specs}$ in the set $\WIN(\Sigma,\Specs)$.

A note: it is common practice in ABCS to ensure safety for sampling times only. This implicitly assumes that sampling times and grid sizes are chosen such that no \enquote{holes} occur between consecutive cells visited in a trajectory. This can be formalized by additional assumptions on the growth rate of $f$ in \eqref{equ:def_f}, which is beyond the scope of our work.

\subsection{Synthesis Using Exhaustive Abstraction}\label{sec:ML_Safety}

This section presents non-lazy abstraction-based safety control before its lazy version is introduced in \REFsec{sec:ML_Safety_Frontier}.

\smallskip
\noindent\textbf{Single-Layered Control}
We consider a 
safety control problem $\tuple{\Sigma,\Specs}$ where $\Specs = \tuple{Y,\Rset{}}$ and recall how it is commonly solved by ABCS for $L=l=1$.
%
In this case one iteratively computes the sets
\begin{equation}\label{equ:safe-fp}
	W^0 = \Rseta{l} \text{ and } W^{i+1} = \FCpre{l}(W^i) \cap \Rseta{l}
\end{equation}
until an iteration $N\in \mathbb{N}$ with $W^N = W^{N+1}$ is reached.
%, where 
%$\FCpre{l}:\twoup{\Xa{l}}\fun\twoup{\Xa{l}}$ is the \emph{controllable predecessor} operator, defined for a set $\Aux\subseteq\Xa{l}$ by
%\begin{equation}
% \FCpre{l}(\Aux) := \set{\xa\in\Xa{l} \mid \exists \ua\in\Ua{}\;.\;\Fa{l}(\xa,\ua) \subseteq \Aux}. \label{eq:define cpre}\\
%\end{equation} 
% This is formalized by the slightly more general procedure $\textproc{CSafe}$ in \REFalg{alg:CSafem}.
% % 
% \begin{algorithm}[]
% 	\caption{Procedure $\textproc{CSafe}$}\label{alg:CSafem}
% 	\begin{algorithmic}[1]
% 	 \Require $\Aux\subseteq \Xa{l}$, $l$
% 	 \State $i\gets 1$
%          \While{$i\leq m$}
% 		\State $\Aux' \gets \FCpre{l}(\Aux) \cap \Aux$\label{alg:CSafem:Iteration}
% 		\If{$\Aux=\Aux'$} 
% 		\State \Return $\Aux$\label{alg:CSafem:FP}
% 		  \Else
% 			  \State $\Aux\gets \Aux'$
% 			  \State $i\gets i+1$
% 		\EndIf
% 	\EndWhile
% 	\State \Return $\Aux$
% 	\end{algorithmic}
% \end{algorithm}
% % 
% It is easy to see that for $m=\infty$ the procedure $\textproc{CSafe}$ computes \eqref{equ:safe-fp} until termination. 
Then $C = (B,\Ua{},G)$ with $B =W^N$, and
\begin{equation}\label{equ:safe-controller}
% 	G(\xa) = \set{\ua\in \Ua{} \mid \Fa{}(\xa,\ua) \subseteq B}
\propImp{\ua\in\Gci{l}(\xa)}{\Fa{l}(\xa,\ua)\subseteq B}
\end{equation}
for all $\xa\in B$, is known to be a safety controller for $\Sa{l}$. 
Then, by the usual argument of FRR between $\Sa{l}$ and $\St{l}$, one can refine the controller $C$ to a sound controller for $\St{l}$.
Note that, even though soundness is guaranteed, completeness is not usually guaranteed; there may exist a state $x\in X$ s.t. $\Qa{l}(x)\not\in \Uc$, and there may exist a controller $C' = (\Uc',\Ua{},G')$, solving the safety control problem $\tuple{\Sigma,\Specs}$ s.t.\ $\Qa{l'}(x)\in \Uc'$ with $l'<l$.


\smallskip
\noindent\textbf{Multi-Layered Control}
Given a sequence of $L$ abstract systems $\Saset:=\set{\Sa{l}}_\layer$ we now present a non-lazy multi-layered ABCS algorithm for safety specifications. We formalize this ABCS procedure by a wrapper function $\MLSAFE(\Rseta{1},L)$, which first calls $\EXPLORE(\UA{l1}(\Rseta{1}),l)$ (see \REFalg{alg:Explore}) for every \layer (eagerly computing the full abstract transitions in all layers) and then calls $\OTFAS(\Rseta{1},\emptyset,L,\emptyset)$.
% 

\begin{algorithm}[t]
	\caption{$\OTFAS$}\label{alg:SafeIt}
	\begin{algorithmic}[1]
		\Require $\Aux\subseteq \Xa{1}$, $\Aux'\subseteq \Xa{1}$, $l$, $\Cset$
% 		\State \textcolor{gray}{$\Aux''\gets\textproc{Frontier}(\Aux',l)$}
% 		\State \textcolor{gray}{$\textproc{Explore}(\UA{l1}(\Aux)\setminus\UA{l1}(\Aux'),l)$}
        \State \fbox{$\EXPLORE{}(\UA{l1}(\Aux)\setminus\UA{l1}(\Aux'),l)$}
\label{alg:SafeIt:Explore}
		\State $W \gets \FCpre{l}(\UA{l1}(\Aux)) \cap \UA{l1}(\Aux)$\label{alg:SafeIt:computeW}
% 		\State $W \gets \textproc{CSafe}(\UA{l1}(\Aux),l)$\label{alg:SafeIt:computeW}
		\State $\Cset\gets\Cset\cup\set{C_l \gets (W,\Ua{},\emptyset)}$\label{alg:SafeIt:safeB}
		\State $\Aux' \gets \Aux'\cup\UA{1l}(W)$\label{alg:SafeIt:safeW}
		\If{$l\neq 1$}
% 			\State $l \gets l-1$
			\State $\OTFAS(\Aux,\Aux',l-1,\Cset)$ // go finer
		\Else
			\If{$\Aux \neq \Aux'$}
% 				\State $\Aux \gets \Aux'$
				\State $\OTFAS(\Aux',\emptyset,L,\emptyset)$ // start new iteration\label{alg:SafeIt:iterate}
			\Else
				\State \Return $\langle \Aux,\Cset \rangle$ // terminate \label{alg:SafeIt:termination}
			\EndIf
		\EndIf
	\end{algorithmic}
\end{algorithm}
% 
%In order to map abstract states between different layers of abstraction, $\textproc{SafeIt}$ uses the operator 
%	\begin{equation}\label{equ:Gamma}
%	 		\UA{ll'}(\Upsilon_{l'}) = 
%			\begin{cases}
%				\Ra{ll'}(\Upsilon_{l'}), & l \leq l' \\
%				\SetComp{\hat{x} \in \Xa{l}}{\Ra{l'l}(\hat{x})\subseteq \Upsilon_{l'}}, & l > l' 
%			\end{cases}
%	\end{equation}
%where $l,l'\in [1;L]$ and $\Upsilon_{l'}\subseteq \Xa{l'}$. 
%The operation $\UA{ll'}(\cdot)$ under-approximates a set of layer $l'$ to a set of layer $l$. 

% \new{As an intermediate step before the lazy version of $\textproc{SafeIt}$ to be presented in \REFsec{sec:ML_Safety_Frontier}, we present a non-lazy version of $\textproc{SafeIt}$ first:}

% Then the set of safe states is computed iteratively by invoking \eqref{equ:safe-fp} for different layers. This is formalized by the wrapper function $\textproc{EagerSafe}$ given in \REFalg{alg:EagerSafe} calling the subroutines $\textproc{Explore}$ and $\textproc{SafeIt}$ given in \REFalg{alg:Explore} and \REFalg{alg:SafeIt}, respectively.
% 
% \begin{algorithm}[]
% 	\caption{Procedure $\textproc{EagerSafe}$}\label{alg:EagerSafe}
% 	\begin{algorithmic}[1]
% 		\Require $\Aux\subseteq \Xa{1}$, $L$
% 		\For {$\layer$} \label{alg:EagerSafe:exploreA}
% 		    \State $\textproc{Explore}(\UA{l1}(\Aux),l)$
% 		\EndFor \label{alg:EagerSafe:exploreB}
%                 \State %$\langle \Aux,\Cset \rangle \gets$
%                 \Return $\textproc{SafeIt}(\Aux,\emptyset,L,\emptyset)$\label{alg:EagerSafe:SafeIt}
% %                 \State \Return $\langle \Aux,\Cset \rangle$
% 	\end{algorithmic}
% \end{algorithm}

% The procedure $\textproc{Explore}$ computes the transition functions in a given abstraction layer $l$ for a specified set of states $\Aux$. Hence, $\textproc{EagerSafe}(\Rseta{1},L)$  After this is done, the iterative function $\textproc{SafeIt}(\Rseta{1},\emptyset,L,\emptyset)$ is called.

\begin{algorithm}[t]
	\caption{$\EXPLORE$ (for $\OTFAS$)}\label{alg:Explore}
	\begin{algorithmic}[1]
		\Require $\Aux\subseteq \Xa{l}$, $l$
		\For {$\xa\in\Aux,\ua\in\Ua$}
		\If {$\Fa{l}(\xa,\ua)$ is undefined}
		\State compute $\Fa{l}(\xa,\ua)$ as in \eqref{eq:next state abs sys 0}
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}
% 

% 
Due to the monotonic nature of the iterative computation of safe sets, the set $\Aux$ in \REFalg{alg:SafeIt} is always a subset of $\Rseta{1}$ (see \REFlem{lem:monotonicity} for a formal treatment). This implies that Line~\ref{alg:SafeIt:Explore} of \REFalg{alg:SafeIt} (boxed) will never perform any exploration (as all needed transition relations are pre-computed) and can therefore be ignored in this section.

When initialized with $\OTFAS{}(\Rseta{1},\emptyset,L,\emptyset)$, \REFalg{alg:SafeIt} performs the following computations: it starts in layer $l=L$ with an outer recursion count $i=1$ (not shown in \REFalg{alg:SafeIt}) and reduces $l$, one step at the time, until $l=1$ is reached, at which point it then starts over again from layer $L$ with $i=i+1$ and a new safe set $\Aux'$. In every such iteration $i$, one step of the safety fixed-point is performed for every layer and the resulting set is stored in the layer $1$ map $\Aux'\subseteq \Xa{1}$, whereas $\Aux\subseteq \Xa{1}$ keeps the knowledge of the previous iteration. If the finest layer is reached and we have $\Aux=\Aux'$, the algorithm terminates. Otherwise $\Aux'$ is copied to $\Aux$, $\Aux'$ and $\Cset$ are reset to $\emptyset$ and $\OTFAS{}$ starts a new iteration (see Line~\ref{alg:SafeIt:iterate}).
% 
After $\OTFAS$ has terminated, it returns a multi-layered controller $\Cset=\set{\Ci{l}}_\layer$ which only contains the domains of the respective controllers $\Ci{l}$ for every layer (see Line~\ref{alg:SafeIt:termination}). The transition functions $\Gci{l}$ can be computed by choosing one input $\ua\in\Ua$ for every $\xa\in \Uci{l}$ s.t.\ 
\begin{equation}\label{def:safecontrollerGci}
 \propImp{\ua=\Gci{l}(\xa)}{\Fa{l}(\xa,\ua)\subseteq \UA{l1}(\Aux)}.
\end{equation}

% It is easy to see that for $m=\infty$, $\textproc{EagerSafe}_\infty$ terminates after one iteration and we essentially recover the safety algortihm presented in \cite{HsuMajumdarMallikSchmuck_HSCC18}, Sec.~.
% % 
% To see the effect of reducing $m$, 

Note that states encountered for layer $l$ in iteration $i$ are saved to the lowest layer $1$ (Line~\ref{alg:SafeIt:safeW} of \REFalg{alg:SafeIt}) and \enquote{loaded} back to the respective layer $l$ in iteration $i+1$ (Line~\ref{alg:SafeIt:computeW} of \REFalg{alg:SafeIt}). Therefore, a state $\xa\in\Xa{l}$ with $l>1$, which was not contained in $W$ as computed in layer $l$ and iteration $i$ via Line~\ref{alg:SafeIt:computeW} of \REFalg{alg:SafeIt}, might still be included in $\UA{l1}(\Aux)$ loaded in the next iteration $i+1$ when re-computing Line~\ref{alg:SafeIt:computeW} for $l$. This happens if all states $x\in\xa$ were added to $\Aux'$ by some layer $l'<l$ in iteration $i$. 
% 
This allows the algorithm to \enquote{bridge} regions that require a finer grid and to use layer $L$ in all remaining regions of the state space. 
% 
The latter is not true for the multi-layered safety algorithm given in \cite[Sec.~4.3]{hsu2018multi} as shown by the example in \cite[Sec.~I-A]{hsu2018lazy}. 


% The lazy computation of the abstract transition systems $\Sa{l}$ for $l<L$ takes place in line~\ref{alg:partial abs}, for all states that need to be explored by the layer $l$ safety fixed-point.


\smallskip
\noindent\textbf{Soundness and Relative Completeness} %\footnote{Absolute completeness of controller synthesis cannot be guaranteed by ABCS; we therefore provide completeness relative to the finest layer.}
Due to the effect described above, the map $W$ encountered in Line~\ref{alg:SafeIt:computeW} for a particular layer $l$ throughout different iterations $i$ might not be monotonically shrinking. However, the latter is true for layer $1$, which is formalized by the following lemma.

\begin{lemma}\label{lem:monotonicity}
 Let $\Aux^0:=\Rseta{1}$ and let $\OTFAS{}$ be called by $\MLSAFE{}(\Rseta{1},L)$, terminating after $N$ iterations. Further, set $\Aux^i:=\Aux'$ whenever \REFalg{alg:SafeIt} reaches Line~\ref{alg:SafeIt:safeW} with $l=1$ for the $i$-th time. Then it holds that $\Aux^i\subseteq\Aux^{i-1}$, hence $\Aux^i\subseteq\Rseta{1}$ for all $i\leq N$.
\end{lemma}

This leads to the following claim, showing that $\MLSAFE{}(\Rseta{1},L)$ is sound and relatively complete.

\begin{theorem}\label{thm:EagerSafe}
Let $\tuple{\Sigma,\Specs}$ be a safety control problem and $\Saset = \set{\Sa{l}}_\layer$ a sequence of abstractions. Let $\langle \Aux^N,\Cset \rangle=\MLSAFE{}(\Rseta{1},L)$ s.t.\ $\Cset=\set{\Ci{l}}_\layer$ and $\Gci{l}$ is defined as in \eqref{def:safecontrollerGci} for all \layer. Further, let $\overline{B}$ be the domain of the single-layer safety controller computed using \eqref{equ:safe-fp} for $l=1$.
Then $\Cset\in\WIN(\Sigma,\Specs)$ and $\overline{B}\subseteq\Aux^N$, i.e. $\Cset$ is sound and relatively complete w.r.t.\ single-layer control for layer $l=1$. 
\end{theorem}


\input{lazySafe}
